Conformal Prediction for Verifiable Learned Query Optimization

Query optimization is critical in relational databases. Recently, numerous Learned Query Optimizers (LQOs) have been proposed, demonstrating superior performance over traditional hand-crafted query optimizers after short training periods. However, the opacity and instability of machine learning models have limited their practical applications. To address this issue, we are the first to formulate the LQO verification as a Conformal Prediction (CP) problem. We first construct the CP model and obtain user-controlled bounded ranges for the actual latency of LQO plans before execution. Then, we introduce CP-based runtime verification along with violation handling to ensure performance prior to execution. For both scenarios, we further extend our framework to handle distribution shifts in the dynamic environment using adaptive CP approaches. Finally, we present CP-guided plan search, which uses actual latency upper bounds from CP to heuristically guide query plan construction. We integrated our verification framework into three LQOs (Balsa, Lero, and RTOS) and conducted evaluations on the JOB and TPC-H workloads. Experimental results demonstrate that our method is both accurate and efficient. Our CP-based approaches achieve tight upper bounds, reliably detect and handle violations. Adaptive CP maintains accurate confidence levels even in the presence of distribution shifts, and the CP-guided plan search improves both query plan quality (up to 9.84x) and planning time, with a reduction of up to 74.4% for a single query and 9.96% across all test queries from trained LQOs.

==> i_sections/background_v1.tex <==
\section{Background}
\label{sec:background}

In this section, we first discuss the granularity levels of prediction decisions to be verified in learned query optimizers (Section~\ref{sec:background_lqo}). Then, we provide a brief introduction for the Conformal Prediction (Section~\ref{sec:background_cp}) and Signal Temporal Logic (Section~\ref{sec:background_stl}) tools that are used to build our verification framework and formally represent the performance constraints we verify {\lqo}s against, respectively.

\subsection{Granularity Levels of Decisions to be Verified in Learned Query Optimizers}
\label{sec:background_lqo}

While Learned Query Optimizers ({\lqo}s) (e.g.,~\cite{neo, bao, balsa,kepler, zhu2023lero, yu2020reinforcement}) can improve the performance over traditional optimizers by adapting to complex queries and data distributions, their reliance on {\ml} models introduces variability and potential unpredictability in performance. Therefore, verifying {\lqo}s against user-defined performance constraints is crucial to ensure that generated plans meet specific efficiency and reliability standards. Broadly, {\lqo}s fall into three categories based on how {\ml} is used. The first category uses {\ml} to improve specific components of the optimizer (e.g., cardinality estimator~\cite{learnedce21,deep_card_est2,neurocard} and cost estimator~\cite{learned_cost_estimator_1,learned_cost_estimator_2}). The second category uses {\ml} to construct the query plan from scratch, replacing the traditional optimizer (e.g.,~\cite{balsa, neo}). The third category uses {\ml} to steer the traditional optimizer in constructing better candidate plans and/or in selecting among them (e.g.,~\cite{bao,zhu2023lero,yu2020reinforcement}). In this paper, we focus on verifying the decisions made by {\lqo}s in the second and third categories only, where {\ml} is involved in constructing the query plan itself. However, the granularity level of these {\lqo} decisions differs between these two categories. In the second category, fine-grained prediction decisions are performed to construct the query plan step-by-step and predict the associated cost at each step. For instance, {\balsa}~\cite{balsa} uses a learned value model to construct the optimized plan operator-by-operator and predict the intermediate cost for the final plan construction at each operator. We refer to the second category as \textit{white-box} {\lqo}s because we rely on these fine-grained prediction decisions during the verification process. In contrast, in the third category, learned models neither perform step-by-step plan construction nor intermediate cost predictions. Instead, they are used to generate useful hints (e.g., determining join orders~\cite{yu2020reinforcement} or hint sets~\cite{bao}) for the traditional optimizer, which then constructs a set of candidate plans. After that, learned models select the best plan from these candidates, either by predicting the high-level cost for each candidate~\cite{bao} or by assigning a relative rank to all candidates~\cite{yu2020reinforcement}. Therefore, in this category, the prediction decisions are mainly only on the level of the whole plan and its high-level associated cost, if available. We refer to the third category as \textit{black-box} {\lqo}s because we only access coarse-grained plan-level decisions (i.e., no sub-plan-level predictions) during the verification process.
 








%In the second category, all {\ml} decisions that are taken to construct the query plan step-by-step, and their associated cost predictions, are available for the verification process. For instance, {\balsa}~\cite{balsa} uses a learned value model to construct the optimized plan operator-by-operator and predict the intermediate cost for the final plan construction at each operator. We refer to the second category as \textit{white-box} {\lqo}s.  In contrast, in the third category, the {\ml} models do not produce step-by-step plan construction or intermediate cost predictions. Instead, they are used to generate useful hints (e.g., determining join orders~\cite{yu2020reinforcement} or hint sets~\cite{bao}) for the traditional optimizer, which then constructs a set of candidate plans. Subsequently, {\ml} models may assist in selecting the best plan from these candidates, either by predicting the high-level cost for each candidate~\cite{bao} or by assigning a relative rank to all candidates~\cite{yu2020reinforcement}. Therefore, in this category, the verification process has access only to the final plan and its high-level cost prediction, if available, which is limited compared to the second category. we refer to the third category as \textit{black-box} {\lqo}s.


%we refer to the third category as \textit{black-box} {\lqo}s because the {\ml} models used in them do not produce step-by-step plan construction or intermediate cost predictions. Instead, {\ml} models generate useful hints (e.g., determining join orders~\cite{yu2020reinforcement} or hint sets~\cite{bao}) for the traditional optimizer, which then constructs a set of candidate plans. Subsequently, {\ml} models may assist in selecting the best plan from these candidates, either by predicting the high-level cost for each candidate~\cite{bao} or by assigning a relative rank to all candidates~\cite{yu2020reinforcement}. In this case, the verification process has access only to the final plan and its high-level cost prediction, if available.

%A query optimizer is a performance-critical component in every database system. It translates declarative user queries into efficient execution plans. Traditional query optimizers, however, often face challenges with effectiveness and efficiency due to the inherent complexity of queries and the variability of data distributions. Consequently, numerous efforts have been made to incorporate machine learning ({\ml}) techniques to address these limitations in query optimization  (e.g.,~\cite{neo, bao, balsa,kepler, zhu2023lero, yu2020reinforcement}). These {\ml}-based approaches can broadly fall into three categories: 1)~using {\ml} to improve specific components of the optimizer (e.g., cardinality estimator~\cite{learnedce21,deep_card_est2,neurocard} and cost estimator~\cite{learned_cost_estimator_1,learned_cost_estimator_2}), 2)~using {\ml} to construct the query plan from scratch, replacing the traditional optimizer (e.g.,~\cite{balsa, neo}), and 3)~using {\ml} to steer the traditional optimizer in constructing better candidate plans and/or in selecting among them (e.g.,~\cite{bao,lero,yu2020reinforcement}). 


\subsection{Conformal Prediction ({\cp})}
\label{sec:background_cp}

We build our {\lqo} verification framework, as shown later, based on Conformal Prediction ({\cp})~\cite{cpbook05,cpgentle23}, a rigorous statistical tool that efficiently quantifies the uncertainty of the {\ml} models' predictions. {\cp} enables users to specify the desired level of confidence in the quantification while being agnostic to the details of the {\ml} models. To introduce {\cp}, assume that \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\) are \(K + 1\) independent and identically distributed (i.i.d) random variables, where each variable \(R^{(i)}\) for \(i \in \{0, \dots, K\}\) is an estimate of the prediction error between the true output \(y^{(i)}\), i.e., ground truth, for input \(x^{(i)}\) and the predicted value of this output $\eta(x^{(i)})$ by the {\ml} predictor~\(\eta\). Formally, this error can be expressed as:
\[
R^{(i)} := \|y^{(i)} - \eta(x^{(i)})\|
\]

\(R^{(i)}\) is commonly referred to as the \textit{non-conformity score}, where a small score suggests a strong predictive model and a large score indicates poorer performance (i.e., less accurate predictions). 

Now, assuming that $R^{(0)}$ belongs to test data and $R^{(1)}, \ldots, R^{(K)}$ are calibration data, the objective of {\cp} is to quantify the uncertainty of \(R^{(0)}\) using \(R^{(1)}, \dots, R^{(K)}\). Specifically, for a user-defined uncertainty probability $\delta \in [0, 1]$ (i.e., $1-\delta$ is a confidence level), {\cp} aims to compute an upper bound $C(R^{(1)}, \dots, R^{(K)})$ for the prediction error $R^{(0)}$ such that:

\[
\text{Prob}(R^{(0)} \leq C(R^{(1)}, \dots, R^{(K)})) \geq 1 - \delta \tag{1}\label{2.2-1}
\]

This upper bound \(C(R^{(1)}, \dots, R^{(K)})\) can be efficiently determined by computing the $(1-\delta)$th quantile of the empirical distribution of $R^{(1)}, \ldots, R^{(K)}$ and $\infty$~\cite{cpgentle23}. For simplicity, we will refer to this upper bound as \(C\) in the rest of the paper. {\cp} guarantees marginal coverage, which is not conditional on the calibration data~\cite{cpgentle23}.



%In both cases, at each step of query plan generation, a predicted cost is computed. This predicted cost quantifies the resources required based on a cost model. Once the plan is generated, it is executed by the query optimizer, and the actual runtime for each step is obtained. These predicted costs and actual runtimes are key performance indicators of the database and form the core of the research presented in this paper.


\subsection{Formal Representation of Performance Constraints to be Verified with {\cp}} 
\label{sec:background_stl}
\todo{Add G notation to STL}
To formally represent the desired performance constraints to verify against {\lqo}s
 (e.g., the execution time of a specific query $\leq$ 100ms), we employ Signal Temporal Logic ({\stl})~\cite{robuststl10}, a {\cp}-compliant formal logical language for verification. {\stl} was originally introduced to verify the properties of time series data (e.g., signals), especially in the context of cyber-physical systems~\cite{stlintro04}. However, it can be used more broadly to accommodate non-traditional time-series data, where the notion of sequence or order still plays an important role. The syntax of an {\stl} specification $\phi$ is recursively defined as $\phi := True \mid \mu \mid \neg \phi \mid \phi \wedge \psi \mid \phi  \mathbf{U}_{[a,b]} \psi$, where $\psi$ is an {\stl} formula. $\neg$, $\wedge$, and $\mathbf{U}_{[a,b]}$ are operators encoding the \textit{not}, \textit{conjunction}, and \textit{until}~\cite{robuststl10} logics that are defined over the {\stl} formulas, respectively.  $\mu$ is a predicate to check whether the specification semantics are achieved or not, i.e., \(\mu: \mathbb{R}^n \to \{\text{True}, \text{False}\}\). \(\mu\) is often defined through a predicate function \( \lambda : \mathbb{R}^n \to \mathbb{R} \) such that \(\mu(x) := \text{True} \) if \( \lambda(x) \geq 0 \) and \(\text{False}\) otherwise, where $\mu(x)$ and $\lambda(x)$ are defined over a sequence of values $x := (x_0, x_1, \ldots)$ and their specification semantics is checked at each value $x_\tau \in x$. If all $x$ values satisfy the constraints represented by $\phi$, we refer to that as $x \models \phi$. 

 

Moreover, we can use \textit{robust} semantics $\rho^{\phi} (x)$, as in~\cite{robuststl09,robuststl10}, to extend the binary evaluation of {\stl} satisfaction (i.e., $\mu(x)$) by providing a quantitative measure of the degree to which this satisfaction is achieved. Unlike traditional binary satisfaction, robust semantics $\rho^{\phi} (x)$ produces a real-valued metric: positive values indicate that the constraint $\phi$ is satisfied, with the magnitude representing the strength of satisfaction, whereas negative values denote a \textit{violation}, with the magnitude reflecting the severity of the violation. For instance, given the constraint \( \phi := x_\tau > 750 \), the robust satisfaction \( \rho^\phi(x) \) can be defined to evaluate \( (x_\tau - 750) \) for each $x_\tau \in x$ and provide a quantitative measure of how robustly all $x$ values  satisfy the condition. More details about robust {\stl} semantics are in~\cite{robuststl09,robuststl10}.


%\(\mu\) is often defined through a predicate function \( \lambda : \mathbb{R}^n \to \mathbb{R} \) such that \(\mu(x, \tau) := \text{True} \) if \( \lambda(x, \tau) \geq 0 \) and \(\text{False}\) otherwise, where $\mu(x, \tau)$ and $\lambda(x, \tau)$ are defined over a sequence of values $x := (x_0, x_1, \ldots)$ and can be calculated at any time~$\tau$ based on $x_\tau \in x$. If all  $x$ values satisfy the constraints represented by $\phi$, we refer to that as $x \models \phi$.

%For instance, given the constraint \( \phi := x_\tau > 750 \), the robust satisfaction can be defined as \( \rho^\phi(x):= (x_\tau - 750) \), providing a quantitative assessment of how robustly the value  \( x_\tau \) satisfies the condition. More details about robust {\stl} semantics are in~\cite{robuststl09,robuststl10}.





==> i_sections/formulation.tex <==
\section{{\cp}-based Latency Guarantees and Runtime Verification for {\lqo} Plans }
\label{sec:problem_formulation}

In this section, we first describe how {\cp} is used to obtain guaranteed latency ranges for the plans generated by {\lqo}s before executing them (Section~\ref{sec:cp_for_lqo}). Then, we show how {\cp} can support runtime verification during the plan construction process, providing guarantees that the evolving plans satisfy user-defined performance constraints (Section~\ref{sec:cp_based_runtime_verification}).


\subsection{{\cp}-based Latency Guarantees for {\lqo}s}
%\subsection{{\lqo}s Prediction Error Analysis using {\cp}}
\label{sec:cp_for_lqo}

%You give an example on the lower value we have for C, the tighter bounds we can get …. 


As mentioned in Section~\ref{sec:background_lqo}, we focus on two categories 
of {\lqo}s: \textit{white-box} and \textit{black-box}, both of which use learned models to construct the query plan itself. In \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}), the learned model builds the query plan incrementally, constructing one partial plan at a time based on a predicted cost (Figure~\ref{fig:lqo_architecture}~(a)). %The predicted cost is designed to reflect the real execution performance of the whole plan when the corresponding sub-plan is used as a step in it: lower costs should correlate with lower execution latency. 
%These partial plans are then assembled into a complete query plan, executed, and its actual latency is used to fine-tune the learned model further. 
Here, we employ {\cp} to obtain \textit{user-controlled guaranteed ranges} for the \textit{actual latency} (not the predicted cost) of these constructed partial plans \textit{before executing them}. For example, given a partial plan $s$ and a user-defined confidence level of 90\%, we can determine a latency range $[l^s_{min}, l^s_{max}]$ that the latency $l^s$ of $s$ will fall within with \textit{at least} 90\% probability, where $l^s_{min}$ and $l^s_{max}$ represent the lower and upper latency bounds, respectively. The intuition is to leverage {\cp} to gain insights into the relationship between predicted costs and actual latencies of partial plans from the {\lqo}'s calibration query workloads, and then use these insights to obtain latency ranges for testing queries. Recall that we assume both calibration and testing queries share the same underlying distribution (check Section~\ref{sec:background_cp}). Therefore, applying calibration-based insights to testing queries is valid. Similarly in \textit{black-box} {\lqo}s (e.g.,~\cite{bao, yu2020reinforcement}), we use {\cp} to provide such user-controlled guaranteed ranges, yet for the end-to-end latencies of complete plans rather than partial ones. This is because \textit{black-box} {\lqo}s rely on learned models solely to select the best plan among complete candidates (Figure~\ref{fig:lqo_architecture}~(b)). %~\footnote{In our {\cp} framework, we consider \textit{black-box} {\lqo}s as a special case of \textit{white-box} {\lqo}s, where the learned model only makes a single, high-level prediction for a large sub-plan at the root.}. 
In the following, we detail our approach to using {\cp} for obtaining these guaranteed latency ranges.



\noindent\textbf{Latency-Cost Non-conformity Score.} A critical step in applying {\cp} is defining the non-conformity score $R$ (check Section~\ref{sec:background_cp}), as it quantifies the deviation between the predicted and actual outcomes. In the {\lqo} context, we focus on how the actual latency of a plan, whether partial or complete, deviates from its predicted cost~\footnote{Note that, during calibration, we can obtain the actual latency of any partial or complete plan straightforwardly with tools like EXPLAIN ANALYZE in PostgreSQL~\cite{postgres_explain_analyze}.}. Following the {\cp} notation, we formally define a \textit{latency-cost non-conformity score} $R^{(i)}$ for the plan at step $\tau$ in any query $q_{j}$ to be:

\[
R^{(i)} := \lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \tag{2}\label{3.1-1}
\]

where $t_{\tau}^{(j)}$ is the actual latency of this plan and $\hat{c}_{\tau}^{(j)}$ is its predicted cost. Note that $R^{(i)}$ represents a score for a calibration plan (i.e., $R^{(i)} \in \{R^{(1)}, \ldots, R^{(K)}\}$) when $q_j$ belongs to the calibration workload $\mathcal{Q}^{Cal}$ and represents a score for a testing plan $R^{(0)}$ when $q_j$ belongs to the testing workload $\mathcal{Q}^{Tst}$ (check Section~\ref{sec:background_cp}). 

%Note that Equation~\ref{3.1-1} can be used to calculate the non-conformity scores of sub-plans in any query $q_j$ belonging to the calibration $\mathcal{Q}^{Cal}$ or testing $\mathcal{Q}^{Tst}$ query workloads.


%Note that Equation~\ref{3.1-1} is used to calculate the calibration $\{R^{(1)}, \ldots, R^{(K)} \}$ and testing $R^{(0)}$ scores, corresponding to the sub-plans in the calibration $\mathcal{Q}^{Cal}$ and  testing $\mathcal{Q}^{Tst}$ query workloads, respectively, i.e., $R^{(i)} \in \{R^{(0)}, R^{(1)}, \ldots, R^{(K)}\}$.


%Formally, assume that $t_{\tau}^{(j)}$ is the actual latency of a sub-plan at step $\tau$ in query $q_{j}$ and $\hat{c}_{\tau}^{(j)}$ is the predicted cost of this sub-plan, then we define a latency-cost non-conformity score $R^{(i)}$ as follows:

%\[
%R^{(i)} := \lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \tag{2}\label{3.1-1}
%\]


%where $R^{(i)} \in \{R^{(0)}, R^{(1)}, \ldots, R^{(K)}\}$ such that $\{R^{(1)}, \ldots, R^{(K)} \}$ is a set of $K$ non-conformity scores defined over all sub-plans of $m$ queries in the calibration workload $\mathcal{Q}^{Cal}$ (i.e., if $q_j \in \mathcal{Q}^{Cal}$), and $R^{(0)}$ is a non-conformity score defined over a sub-plan of a query in the testing workload $\mathcal{Q}^{Tst}$ (i.e., if $q_j \in \mathcal{Q}^{Tst}$).

%%%TODO: maybe we should say R = |t-funct(c)| and func is for normalization
%%%TODO: Put an example here for these  different sub-plans from queries and 

\noindent\textbf{Guaranteed Range of Plan Actual Latency.} Using equations \ref{2.2-1} and~\ref{3.1-1}, we can directly derive an upper bound~\(C\) on the latency-cost non-conformity score of any plan, whether partial or complete, in a testing query such that:

\[
P(\lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \leq C) \geq 1 - \delta \label{4.3-1}\tag{3}
\]

By reformulating Equation~\ref{4.3-1}, we can compute a range for the actual latency $t_{\tau}^{(j)}$ of this plan, with confidence \(1 - \delta\), based on its predicted cost $\hat{c}_{\tau}^{(j)}$ and the upper bound \(C\) as follows:

\[
P(\hat{c}_{\tau}^{(j)} - C \leq t_{\tau}^{(j)} \leq \hat{c}_{\tau}^{(j)} + C) \geq 1 - \delta \label{4.3-2}\tag{4}
\]
 
This allows us to estimate a \textit{guaranteed} range for the actual latency even prior to executing the plan. However, the tightness of this range primarily depends on the upper bound~\(C\), which itself is influenced by the number of calibration plans used to establish it. Therefore, determining the sufficient number of calibration plans to construct a valid upper bound~\(C\) is crucial. Here, we derive a lower bound on this number: \\


%as the $(1-\delta)$th quantile of the empirical distribution of the $K$ non-conformity scores of calibration sub-plans $R^{(1)}, \ldots, R^{(K)}$ and $\infty$, assuming the availability of independent $\mathcal{Q}^{Tra}$ and $\mathcal{Q}^{Cal}$ query workloads (and their sub-plans latencies) for training and calibrating the {\lqo}, respectively



\vspace{-8pt}

 \textbf{Lemma~1} \textbf{(Lower Bound on Required Calibration Plans)}. \textit{Let the latency-cost non-conformity scores of a testing plan $R^{(0)}$ and $K$ calibration plans $R^{(1)}, \ldots, R^{(K)}$ be exchangeable and realizing i.i.d random variables, $\delta \in [0, 1]$ be a user-defined uncertainty probability, and $C$ be an upper bound on the score $R^{(0)}$ of the testing plan, calculated at a confidence level of $1-\delta$. Then, the lower bound on the number of calibration plans, i.e., $K$, to calculate $C$ is $\frac{1 - \delta}{\delta}$.}\\

\vspace{-8pt}

 \textbf{Proof.} If the scores $R^{(0)}, R^{(1)}, \ldots, R^{(K)}$ are exchangeable (i.e., independent of their order and are drawn from the same distribution), then the joint distribution of these scores remains unchanged~\cite{cpgentle23}. This means that the rank of any score, including $R^{(0)}$, is \textit{uniformly} distributed on the ranks $\{1, \ldots, K+1\}$. As a result, we can estimate the probability of the $R^{(0)}$'s rank in this uniform distribution using the $1-\delta$ quantile as follows:

\[
\text{Prob} (\text{Rank of } R^{(0)} \leq \lceil (K + 1)(1 - \delta) \rceil) \geq 1 - \delta
\]

where \(\lceil \cdot \rceil\) denoting the ceiling function. However, according to~\cite{cpgentle23}, if \(\lceil (K+1)(1-\delta) \rceil > K\), then the upper bound \(C\) becomes trivial and uninformative, yielding \(C = \infty\). Therefore, to ensure that \(C\) is nontrivial, we need the following condition: 

\[\lceil (K+1)(1-\delta) \rceil \leq K\]

From this, we can easily get \(K \geq \frac{1 - \delta}{\delta}\), which means the lower bound on the number of calibration plans should be $\frac{1 - \delta}{\delta}$.

%%% TODO: show some examples with delta 0.1 or 0.05





%\textbf{Marginal Coverage Guarantees.} We would like to highlight that the guarantee in the equation is marginal, referring to the randomness across both the test and calibration data points \(R^{(0)}, R^{(1)},\\ \dots, R^{(K)}\), rather than conditional on the specific values of the calibration set \(R^{(1)}, \dots, R^{(K)}\). In other words, \(\text{Prob}(\cdot)\) reflects the randomness arising from the draw over all random variables. 

%Based on the previous discussion, we conclude the core formula we use in our framework as follows:
%\[
%P(\lVert t^{(i)} - \hat{c}^{(i)} \rVert \leq C) \geq 1 - \delta. \tag{5}\label{eq:5}
%\]
%where \(i\) means the data point index in our data series. We construct \(C\) based on the calibration set and then apply this \(C\) and \(\delta\) to other data points to provide the same guarantees. In our framework, this conformal prediction formula offers us guarantees with confidence.


\subsection{{\cp}-based Runtime Verification for White-Box {\lqo}s Plan Construction}
\label{sec:cp_based_runtime_verification}




Earlier (Section~\ref{sec:cp_for_lqo}), we showed how {\cp} can provide a guaranteed latency range for partial or complete query plans, helping assess the uncertainty of {\lqo} decisions before execution. Here, we aim to go further by exploring the use of {\cp} to early detect any performance constraint violations during the plan construction process of \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}), based solely on the constructed partial plans so far and before the full plan is completed. 

Suppose \(\mathcal{D}\) is an unknown distribution over the query plans generated by a white-box {\lqo}. Let \(X := (X_0, X_1, \dots) \sim \mathcal{D}\) represent a random query plan generated by the {\lqo}, where \(X_{\tau}\) is a random variable denoting the state of the generated partial plan at step~$\tau$ (e.g., predicted cost or actual latency). Then, we can formally define the white-box {\lqo} runtime verification problem as follows:\\

%Also, assume the availability of independent $\mathcal{Q}^{Tra}$ and $\mathcal{Q}^{Cal}$ query workloads for training and calibrating the {\lqo}, respectively.

\vspace{-8pt}

\textbf{Definition~1 (The White-Box {\lqo} Runtime Verification Problem).} \textit{Assuming a white-box {\lqo} (e.g.,~\cite{balsa}) and a testing query~$q$ that this {\lqo} already finished constructing its partial plans till step $\tau$ and is still running, we aim to \underline{verify} whether all generated partial plans by this {\lqo} (past and future) result in a complete plan, represented by $X$, that satisfies a user-defined STL-based performance constraint~$\phi$ with a confidence level $1-\delta$, i.e., $\text{Prob} (X \models \phi) \geq 1 - \delta$, where $\delta \in [0, 1]$ is a constraint violation probability.} \\

\vspace{-8pt}

Let \(x:= (x_0, x_1, \ldots)\) be the realization of \(X := (X_0, X_1, \dots)\), where \(x_{\text{obs}} := (x_0, \ldots, x_\tau)\) represents the constructed partial plans till step $\tau$ and \(x_{\text{un}} := (x_{\tau+1}, x_{\tau+2}, \ldots)\) represents the future unknown partial plans that will be predicted. Since existing \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}) predict one partial plan at a time, then we can estimate the realization $x$ at step $\tau$, with its constructed plans so far (i.e., $x_{\text{obs}}$) and next prediction at step $\tau+1$ as follows:

\[
\hat{x} := (x_{\text{obs}}, \hat{x}_{\tau+1 \mid \tau}) \label{3.2-1}\tag{5}
\]


As described in Definition~1, our goal is to verify the quality of the white-box {\lqo}'s complete query plan, represented by $X$, against a user-defined {\stl} specification \(\phi\). We can use robust semantics \(\rho^\phi(.)\) (check Section~\ref{sec:background_stl}) to achieve that. First, we define \(\rho^\phi(X)\) to indicate how robustly the specification \(\phi\) is satisfied with the complete query plan, and \(\rho^\phi(\hat{x})\) to denote the estimate of this robustness we obtained so far based on the observations \(x_{\text{obs}}\) and the prediction \(\hat{x}_{\tau+1 \mid \tau}\). Then, according to~\cite{cpstl23,prtstl23}, we can use {\cp} (Equation~\ref{2.2-1}) to define an upper bound \(C\) on the difference between the actual robustness \(\rho^\phi(X)\) of the complete query and the estimate of this robustness \(\rho^\phi(\hat{x})\) till step $\tau$ such that:  

\[
\text{Prob}(\rho^\phi(\hat{x}) - \rho^\phi(X) \leq C) \geq 1 - \delta \tag{6}\label{3.2-2}
\]

This upper bound \(C\) can be easily obtained from the calibration query workload $\mathcal{Q}^{Cal}$ by calculating the following non-conformity score $R^{(i)}$ for each partial plan in each calibration query $q_i \in \mathcal{Q}^{Cal}$:

\[
R^{(i)} := \rho^\phi(\hat{x}^{(i)}) - \rho^\phi(x^{(i)}) \label{3.2-3}\tag{7}
\]

where $x^{(i)}$ is the realization of $X$ for query $q_i$ (i.e., actual latencies and predicted costs for all partial plans in $q_i$) and \(\hat{x}^{(i)}\) is the estimate of this realization till step $\tau$ only (i.e., \(\hat{x}^{(i)} := (x_{\text{obs}}^{(i)}, \hat{x}_{\tau+1 \mid \tau}^{(i)})\)). Given that, we can define the following condition to verify whether the {\lqo} satisfies $\phi$ or not:\\

\vspace{-8pt}

\textbf{Lemma~2 (The White-Box {\lqo} Runtime Verification Condition).} \textit{Given a testing query $q$ that uses {\lqo} to generate its plan, represented by \(X\), and with $\hat{x} := (x_{\text{obs}}, \hat{x}_{\tau+1 \mid \tau})$ realizing the constructed and predicted partial plans at step $\tau$, an {\stl} constraint $\phi$, a robust semantics measure \(\rho^\phi(.)\) for this $\phi$ constraint, and a constraint violation probability $\delta \in [0, 1]$. Then, we can \underline{guarantee} that these constructed and predicted partial plans $\hat{x}$ so far will result in a complete plan that satisfies the constraint $\phi$ with a confidence level $1-\delta$, i.e., $\text{Prob} (X \models \phi) \geq 1 - \delta$, only if the robust semantics defined over these partial plans \underline{$\rho^\phi(\hat{x})$ is larger than $C$}, where $C$ is an upper bound calculated at a confidence level $1-\delta$ and using equations~\ref{3.2-2} and~\ref{3.2-3}. Otherwise, the resulting complete plan will cause a violation.}\\

\vspace{-8pt}


\textbf{Proof.} By reformulating Equation~\ref{3.2-2}, we can obtain:
\[
P(\rho^\phi(X) \geq \rho^\phi(\hat{x}) - C) \geq 1 - \delta\label{3.2-4}\tag{8}
\]
If \(\rho^\phi(\hat{x}) > C\), it implies:
\[
P(\rho^\phi(X) > 0) \geq 1 - \delta\label{3.2-5}\tag{9}
\]
which, according to Section~\ref{sec:background_stl}, further implies:
\[
P(X \models \phi) \geq 1 - \delta\label{3.2-6}\tag{10}
\]
because \(\rho^\phi(X) > 0\) directly implies that \(X \models \phi\). Note that changing the constraint specification \(\phi\) and/or the robust semantics measure \(\rho^\phi(.)\) does not require retraining the white-box {\lqo} to obtain valid guarantees because its prediction decisions, i.e., partial plans, are agnostic to any constraint specification.  



 
 
 

 


==> i_sections/formulation_v1.tex <==
\section{{\cp}-based Latency Guarantees and Runtime Verification for {\lqo} Plans }
\label{sec:problem_formulation}

In this section, we first describe how {\cp} is used to obtain guaranteed latency ranges for the plans generated by {\lqo}s before executing them (Section~\ref{sec:cp_for_lqo}). Then, we show how {\cp} can support runtime verification during the plan construction process, providing guarantees that the evolving plans satisfy user-defined performance constraints (Section~\ref{sec:cp_based_runtime_verification}).


\subsection{{\cp}-based Latency Guarantees for {\lqo}s}
%\subsection{{\lqo}s Prediction Error Analysis using {\cp}}
\label{sec:cp_for_lqo}

As mentioned in Section~\ref{sec:background_lqo}, we focus on two categories 
of {\lqo}s: \textit{white-box} and \textit{black-box}, both of which use learned models to construct the query plan itself. In \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}), the learned model builds the query plan incrementally, constructing one sub-plan at a time and predicting its associated cost. %The predicted cost is designed to reflect the real execution performance of the whole plan when the corresponding sub-plan is used as a step in it: lower costs should correlate with lower execution latency. 
These sub-plans are then assembled into a complete query plan, executed, and its actual latency is used to fine-tune the learned model further. We aim to use {\cp} to obtain \textit{guaranteed ranges} of the actual latency in these constructed sub-plans before executing them. Similarly in \textit{black-box} {\lqo}s (e.g.,~\cite{bao, yu2020reinforcement}), we use {\cp} to have such guaranteed ranges, yet on the complete plan only, and its high-level predicted latency if available, as sub-plan-level predictions are not applicable~\footnote{In our {\cp} framework, we consider \textit{black-box} {\lqo}s as a special case of \textit{white-box} {\lqo}s, where the learned model only makes a single, high-level prediction for a large sub-plan at the root.}. 
In the following, we introduce how we effectively use {\cp} with {\lqo}s to obtain these guaranteed ranges.

%%%% TODO: an example of the partial planning if needed %%%%%%% 

\noindent\textbf{Latency-Cost Non-conformity Score.} A critical step in applying {\cp} is defining the non-conformity score $R$ (check Section~\ref{sec:background_cp}), as it quantifies the deviation between the predicted and actual outcomes. In the {\lqo} context, we focus on how the actual latency of running a sub-plan deviates from its predicted cost \footnote{Note that we can obtain the actual latency of each sub-plan straightforwardly with tools like EXPLAIN ANALYZE in PostgreSQL~\cite{postgres_explain_analyze}.}. Following the {\cp} notation in Section~\ref{sec:background_cp}, we formally define a \textit{latency-cost non-conformity score} $R^{(i)}$ for a sub-plan at step $\tau$ in query $q_{j}$ to be:

\[
R^{(i)} := \lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \tag{2}\label{3.1-1}
\]

where $t_{\tau}^{(j)}$ is the actual latency of this sub-plan and $\hat{c}_{\tau}^{(j)}$ is its predicted cost. Note that Equation~\ref{3.1-1} can be used to calculate the non-conformity scores of sub-plans in any query $q_j$ belonging to the calibration $\mathcal{Q}^{Cal}$ or testing $\mathcal{Q}^{Tst}$ query workloads.


%Note that Equation~\ref{3.1-1} is used to calculate the calibration $\{R^{(1)}, \ldots, R^{(K)} \}$ and testing $R^{(0)}$ scores, corresponding to the sub-plans in the calibration $\mathcal{Q}^{Cal}$ and  testing $\mathcal{Q}^{Tst}$ query workloads, respectively, i.e., $R^{(i)} \in \{R^{(0)}, R^{(1)}, \ldots, R^{(K)}\}$.


%Formally, assume that $t_{\tau}^{(j)}$ is the actual latency of a sub-plan at step $\tau$ in query $q_{j}$ and $\hat{c}_{\tau}^{(j)}$ is the predicted cost of this sub-plan, then we define a latency-cost non-conformity score $R^{(i)}$ as follows:

%\[
%R^{(i)} := \lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \tag{2}\label{3.1-1}
%\]


%where $R^{(i)} \in \{R^{(0)}, R^{(1)}, \ldots, R^{(K)}\}$ such that $\{R^{(1)}, \ldots, R^{(K)} \}$ is a set of $K$ non-conformity scores defined over all sub-plans of $m$ queries in the calibration workload $\mathcal{Q}^{Cal}$ (i.e., if $q_j \in \mathcal{Q}^{Cal}$), and $R^{(0)}$ is a non-conformity score defined over a sub-plan of a query in the testing workload $\mathcal{Q}^{Tst}$ (i.e., if $q_j \in \mathcal{Q}^{Tst}$).

%%%TODO: maybe we should say R = |t-funct(c)| and func is for normalization
%%%TODO: Put an example here for these  different sub-plans from queries and 

\noindent\textbf{Guaranteed Range of Sub-plan Actual Latency.} Using equations \ref{2.2-1} and~\ref{3.1-1}, we can directly derive an upper bound~\(C\) on the latency-cost non-conformity score of any sub-plan in a testing query such that:

\[
P(\lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert \leq C) \geq 1 - \delta \label{4.3-1}\tag{3}
\]

By reformulating Equation~\ref{4.3-1}, we can compute a range for the actual latency $t_{\tau}^{(j)}$ of this sub-plan, with confidence \(1 - \delta\), based on its predicted cost $\hat{c}_{\tau}^{(j)}$ and the upper bound \(C\) as follows:

\[
P(\hat{c}_{\tau}^{(j)} - C \leq t_{\tau}^{(j)} \leq \hat{c}_{\tau}^{(j)} + C) \geq 1 - \delta \label{4.3-2}\tag{4}
\]
 
This allows us to estimate a \textit{guaranteed} range for the actual latency even prior to executing the sub-plan. However, the tightness of this range primarily depends on the upper bound~\(C\), which itself is influenced by the number of calibration sub-plans used to establish it. Therefore, determining the sufficient number of calibration sub-plans to construct a valid upper bound~\(C\) is crucial. Here, we derive a lower bound on this number: \\


%as the $(1-\delta)$th quantile of the empirical distribution of the $K$ non-conformity scores of calibration sub-plans $R^{(1)}, \ldots, R^{(K)}$ and $\infty$, assuming the availability of independent $\mathcal{Q}^{Tra}$ and $\mathcal{Q}^{Cal}$ query workloads (and their sub-plans latencies) for training and calibrating the {\lqo}, respectively



\vspace{-8pt}

 \textbf{Lemma~1} \textbf{(Lower Bound on Required Calibration Sub-plans)}. \textit{Let the latency-cost non-conformity scores $R^{(0)}, R^{(1)}, \ldots, R^{(K)}$ be exchangeable~\cite{cpgentle23} and realizing i.i.d random variables, $\delta \in [0, 1]$ be a user-defined uncertainty probability, and $C$ be an upper bound on the score $R^{(0)}$ of any testing sub-plan, calculated at a confidence level of $1-\delta$. Then, the lower bound on the number of required calibration sub-plans, i.e., $K$, to calculate $C$ is $\frac{1 - \delta}{\delta}$.}\\

\vspace{-8pt}

 \textbf{Proof.} If the scores $R^{(0)}, R^{(1)}, \ldots, R^{(K)}$ are exchangeable (i.e., independent of their order and are drawn from the same distribution), then the joint distribution of these scores remains unchanged~\cite{cpgentle23}. This means that the rank of any score, including $R^{(0)}$, is \textit{uniformly} distributed on the ranks $\{1, \ldots, K+1\}$. As a result, we can estimate the probability of the $R^{(0)}$'s rank in this uniform distribution using the $1-\delta$ quantile as follows:

\[
\text{Prob} (\text{Rank of } R^{(0)} \leq \lceil (K + 1)(1 - \delta) \rceil) \geq 1 - \delta
\]

where \(\lceil \cdot \rceil\) denoting the ceiling function. However, according to~\cite{cpgentle23}, if \(\lceil (K+1)(1-\delta) \rceil > K\), then the upper bound \(C\) becomes trivial and uninformative, yielding \(C = \infty\). Therefore, to ensure that \(C\) is nontrivial, we need the following condition: 

\[\lceil (K+1)(1-\delta) \rceil \leq K\]

From this, we can easily get \(K \geq \frac{1 - \delta}{\delta}\), which means the lower bound on the number of calibration sub-plans should be $\frac{1 - \delta}{\delta}$.

%%% TODO: show some examples with delta 0.1 or 0.05





%\textbf{Marginal Coverage Guarantees.} We would like to highlight that the guarantee in the equation is marginal, referring to the randomness across both the test and calibration data points \(R^{(0)}, R^{(1)},\\ \dots, R^{(K)}\), rather than conditional on the specific values of the calibration set \(R^{(1)}, \dots, R^{(K)}\). In other words, \(\text{Prob}(\cdot)\) reflects the randomness arising from the draw over all random variables. 

%Based on the previous discussion, we conclude the core formula we use in our framework as follows:
%\[
%P(\lVert t^{(i)} - \hat{c}^{(i)} \rVert \leq C) \geq 1 - \delta. \tag{5}\label{eq:5}
%\]
%where \(i\) means the data point index in our data series. We construct \(C\) based on the calibration set and then apply this \(C\) and \(\delta\) to other data points to provide the same guarantees. In our framework, this conformal prediction formula offers us guarantees with confidence.


\subsection{{\cp}-based Runtime Verification for {\lqo}s}
\label{sec:cp_based_runtime_verification}

Earlier (Section~\ref{sec:cp_for_lqo}), we showed how {\cp} can provide a guaranteed latency range for partial or complete query plans, helping assess the uncertainty of {\lqo} decisions before execution. Here, we aim to go further by exploring the use of {\cp} to perform runtime verification throughout the plan construction process in \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}), enabling early detection of performance constraint violations based solely on the constructed sub-plans so far and before the full plan is completed.

Suppose \(\mathcal{D}\) is an unknown distribution over the query plans generated by {\lqo}. Let \(X := (X_0, X_1, \dots) \sim \mathcal{D}\) represents a random query plan generated by {\lqo}, where \(X_{\tau}\) is a random variable denoting the state of the generated sub-plan at step $\tau$ (e.g., predicted cost or actual latency of the sub-plan). Also, assume the availability of independent $\mathcal{Q}^{Tra}$ and $\mathcal{Q}^{Cal}$ query workloads for training and calibrating the {\lqo}, respectively. Then, we can formally define the {\lqo} runtime verification problem as follows:\\

\vspace{-8pt}

\textbf{Definition~1 (The {\lqo} Runtime Verification Problem).} \textit{Assuming a {\lqo} (e.g.,~\cite{balsa}), which is trained and calibrated with $\mathcal{Q}^{Tra}$ and $\mathcal{Q}^{Cal}$, respectively, and a testing query $q$ that {\lqo} already finished constructing its sub-plans till step $\tau$ and is still running, we aim to \underline{verify} whether all generated sub-plans by {\lqo} (past and future) result in a complete plan, represented by $X$, that satisfies user-defined {\stl} constraint $\phi$ with a confidence level $1-\delta$, i.e., $\text{Prob} (X \models \phi) \geq 1 - \delta$, where $\delta \in [0, 1]$ is a constraint violation probability.} \\

\vspace{-8pt}

Let \(x:= (x_0, x_1, \ldots)\) be the realization of \(X := (X_0, X_1, \dots)\), where \(x_{\text{obs}} := (x_0, \ldots, x_\tau)\) represents the constructed sub-plans till step $\tau$ and \(x_{\text{un}} := (x_{\tau+1}, x_{\tau+2}, \ldots)\) represents the future unknown sub-plans that will be predicted. Since existing \textit{white-box} {\lqo}s (e.g.,~\cite{balsa, neo}) predict one sub-plan at a time, then we can estimate the realization $x$ at step $\tau$, with its constructed plans so far (i.e., $x_{\text{obs}}$) and next prediction at step $\tau+1$ as follows:

\[
\hat{x} := (x_{\text{obs}}, \hat{x}_{\tau+1 \mid \tau}) \label{3.2-1}\tag{5}
\]

As described in Definition~1, our goal is to verify the quality of the {\lqo}'s complete query plan, represented by $X$, against a user-defined {\stl} specification \(\phi\). We can use robust semantics \(\rho^\phi(.)\) (check Section~\ref{sec:background_stl}) to achieve that. First, we define \(\rho^\phi(X)\) to indicate how robustly the specification \(\phi\) is satisfied with the complete query plan, and \(\rho^\phi(\hat{x})\) to denote the estimate of this robustness we obtained so far based on the observations \(x_{\text{obs}}\) and the prediction \(\hat{x}_{\tau+1 \mid \tau}\). Then, according to~\cite{cpstl23,prtstl23}, we can use {\cp} (Equation~\ref{2.2-1}) to compute an upper bound \(C\) on the difference between the actual robustness \(\rho^\phi(X)\) and its estimate \(\rho^\phi(\hat{x})\) such that:  

\[
\text{Prob}(\rho^\phi(\hat{x}) - \rho^\phi(X) \leq C) \geq 1 - \delta \tag{6}\label{3.2-2}
\]

We can obtain this upper bound \(C\) from the calibration query workload $\mathcal{Q}^{Cal}$ by calculating the following non-conformity score $R^{(i)}$ over the sub-plans in each calibration query (\(x^{(i)} \in \mathcal{Q}^{Cal}\)):

\[
R^{(i)} := \rho^\phi(\hat{x}^{(i)}) - \rho^\phi(x^{(i)}) \label{3.2-3}\tag{7}
\]

where \(\hat{x}^{(i)} := (x_{\text{obs}}^{(i)}, \hat{x}_{\tau+1 \mid \tau}^{(i)})\). Given that, we can define the following condition to verify whether the {\lqo} satisfies $\phi$ or not:\\

\vspace{-8pt}

\textbf{Lemma~2 (The {\lqo} Runtime Verification Condition).} \textit{Given a testing query $q$ that uses {\lqo} to generate its plan, represented by \(X\), and with $\hat{x} := (x_{\text{obs}}, \hat{x}_{\tau+1 \mid \tau})$ realizing the constructed and predicted sub-plans at step $\tau$, an {\stl} constraint $\phi$, a robust semantics measure \(\rho^\phi(.)\) for this $\phi$ constraint, and a constraint violation probability $\delta \in [0, 1]$. Then, we can \underline{guarantee} that these constructed and predicted sub-plans $\hat{x}$ so far will result in a complete plan that satisfies the constraint $\phi$ with a confidence level $1-\delta$, i.e., $\text{Prob} (X \models \phi) \geq 1 - \delta$, only if the robust semantics defined over these sub-plans \(\rho^\phi(\hat{x}) > C\), where $C$ is an upper bound calculated using equations~\ref{3.2-2} and~\ref{3.2-3}. Otherwise, the resulting complete plan will cause a violation.}\\

\vspace{-8pt}


\textbf{Proof.} By reformulating Equation~\ref{3.2-2}, we can obtain:
\[
P(\rho^\phi(X) \geq \rho^\phi(\hat{x}) - C) \geq 1 - \delta\label{3.2-4}\tag{8}
\]
If \(\rho^\phi(\hat{x}) > C\), it implies:
\[
P(\rho^\phi(X) > 0) \geq 1 - \delta\label{3.2-5}\tag{9}
\]
which, according to Section~\ref{sec:background_stl}, further implies:
\[
P(X \models \phi) \geq 1 - \delta\label{3.2-6}\tag{10}
\]
because \(\rho^\phi(X) > 0\) directly implies that \(X \models \phi\). Note that changing the constraint specification \(\phi\) and/or the robust semantics measure \(\rho^\phi(.)\) does not require retraining the {\lqo} to obtain valid guarantees because its prediction decisions, i.e., sub-plans, are agnostic to any constraint specification.  



 
 
 

 


==> sections/background.tex <==
\section{Background (1 page)}
\subsection{Learned Query Optimizer (0.6 column)}
\hanwen{Balsa Details: the things we need to integrate our system; separate branches}
Query optimizers translate SQL queries into efficient query plans. Recently, learned query optimizers have leveraged machine learning models to generate better query plans. These learned query optimizers can be broadly categorized into two branches. The first branch constructs query plans operator by operator, with each step influenced by the machine learning model’s predictions. We refer to this approach as direct and transparent to the system. The second branch, which is indirect, uses machine learning to determine join orderings (without generating an exact plan) or selects the best plan from a set of candidate plans by comparing their quality in a pairwise manner.

In both cases, at each step of query plan generation, a predicted cost is computed. This predicted cost quantifies the resources required based on a cost model. Once the plan is generated, it is executed by the query optimizer, and the actual runtime for each step is obtained. These predicted costs and actual runtimes are key performance indicators of the database and form the core of the research presented in this paper.

\subsection{Conformal Prediction}
Consider the following scenario, given \(K + 1\) independent and identically distributed random variables \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\), conformal prediction aims to measure the uncertainty of \(R^{(0)}\) using \(R^{(1)}, \dots, R^{(K)}\).Specifically, for a given failure probability \(\delta \in (0,1)\), our objective is to construct a probabilistically valid prediction region \(C : \mathbb{R}^K \to \mathbb{R}\), such that:
\[
\text{Prob}(R^{(0)} \leq C(R^{(1)}, \dots, R^{(K)})) \geq 1 - \delta. \tag{1}\label{2.2-1}
\]

Equation (\ref{2.2-1}) allows us to compute a probabilistic upper bound for a test sample \(R^{(0)}\) based on the calibration dataset \(R^{(1)}, \dots, R^{(K)}\). Conformal prediction offers a straightforward and efficient method to calculate the upper bound \(C(R^{(1)}, \dots, R^{(K)})\), ensuring that it holds with a confidence level of \(1 - \delta\). For simplicity, we will refer to this upper bound as \(C\) in the following discussion. 

The variable \(R^{(i)}\) for \(i \in \{0, \dots, K\}\) is commonly referred to as the nonconformity score. In the context of regression, it is often defined as the prediction error, given by:
\[
R^{(i)} := \|y^{(i)} - \mu(x^{(i)})\|,
\]
where a predictor \(\mu\) attempts to predict based on the input \(x^{(i)}\) and \(y^{(i)}\) is the ground truth. A small nonconformity score suggests a strong predictive model, while a large score indicates poorer performance. 


% Let us assume the underlying model is a classification problem, we can apply a similar approach to regression problems, which we discuss in subsequent sections. Consider a classification problem with $K$ classes and a function $\hat{f}(X)$ that predicts one of these classes given an input \(X\). To integrate a conformal predictor, we first create a new dataset, called the calibration dataset, which remains unseen during the training phase. This calibration dataset is essential for assessing the model's performance and computing conformal scores that reflect the uncertainty of the predictions.
% Using this calibration dataset, we calculate the conformal scores for each prediction. To quantify 
% the prediction score we can use the softmax score of the predictions.
% \begin{equation}
%     \mu_i = |Y_i - \hat{Y}_i|
% \end{equation} 
% $\mu$ is known as the nonconformity score. A low (high) nonconformity score indicates a good (poor) model performance. These scores measure how well each prediction fits within the context of the calibration data, providing a basis for determining the confidence in each prediction.\\
% The next step involves computing the nonconformity quantile corresponding to the significance level $\delta \in (0,1)$ , which represents the desired confidence level. 
% \begin{equation}
%     \hat{q} = \frac{\lceil(n+1)(1-\delta)\rceil}{n}
% \end{equation}
% Where $n$ indicates the size of the dataset and the $\lceil . \rceil$ is the ceil operation. This quantile value acts as a threshold for selecting the predictions that will be included in the final prediction set. A class is included in the prediction set if its softmax score is greater than $1-\delta$. We move to the test dataset, where we construct a prediction region for every input. This prediction set consists of all classes whose conformal scores exceed \(1 - \delta\). By including only these classes, we ensure that the prediction region maintains the desired level of confidence, effectively managing the uncertainty in the model's predictions.\\
% \begin{equation}
%     P(Y_{true} \in C(X_{test})) > 1-\delta 
% \end{equation} 
% This method not only provides a robust mechanism for uncertainty quantification in classification problems but also enhances the reliability of the predictions by incorporating a formal, statistically grounded approach. The ability to control the confidence level through \(\delta\) offers flexibility and adaptability, making the conformal prediction framework a valuable tool in various practical applications.\\
% Extrapolating a similar concept for regression problems. The $\hat{q}$ would be the difference between predicted and actual values. We can convert a point prediction to a range prediction to attain confidence levels.
% \begin{equation}
%     P(Y_{true} \in [\hat{f}(X_{test}) - \hat{q}, \hat{f}(X_{test}) + \hat{q}]) > 1 - \delta
% \end{equation}



% [Original Text, Already Rewritten] Suppose \(D\) is an unknown distribution over trajectories that describe our system's behaviors. let \(X := (X_0, X_1, \dots) \sim \mathcal{D}\) be a random trajectory where \(X_{\tau}\) denotes the state of the system at time \(\tau\) that is drawn from \(\mathbb{R}^n\). \((x_0, x_1, \ldots)\) denotes a realization of \(X := (X_0, X_1, \ldots) \sim D\). Assume that we have observed \(x_{\text{obs}} := (x_0, \ldots, x_t)\) at time \(t\), i.e., all states up until time \(t\) are known, while the realizations of \(x_{\text{un}} := (x_{t+1}, x_{t+2}, \ldots)\) are not known yet. Consequently, we have that \(X := (X_{\text{obs}}, X_{\text{un}})\). In this paper, we are interested in calculating the probability that \((X, \tau_0) \models \phi\) as formally stated next.

% [Original Text, Already Rewritten] \paragraph{\textbf{Problem 1}}
% Given a distribution \((X_0, X_1, \ldots) \sim D\), the current time \(t\), the observations \(x_{\text{obs}} := (x_0, \ldots, x_t)\), a bounded STL formula \(\phi\) that is enabled at \(\tau_0\), and a failure probability \(\delta \in (0, 1)\), determine if \(P((X, \tau_0) \models \phi) \geq 1 - \delta\) holds.

% [Original Text, Already Rewritten] We first propose a solution by a direct application of conformal prediction. Let us therefore define \(H := \tau_0 + L^\phi - t\) as the maximum prediction horizon that is needed to estimate the satisfaction of the bounded STL specification \(\phi\). Define now the predicted trajectory
% \[
% \hat{x} := (x_{\text{obs}}, \hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t})
% \]


%%[Rewrite on Oct9] We propose a solution by applying conformal prediction directly. To begin, define \(H := \tau_0 + L^\phi - t\) as the maximum prediction horizon required to estimate the satisfaction of the bounded STL specification \(\phi\). Now, define the predicted trajectory as follows:
% \[
% \hat{x} := (x_{\text{obs}}, \hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t})
% \]
%[Rewrite on Oct9]which is the concatenation of the current observations \(x_{\text{obs}}\) and the predictions of future states \(\hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t}\). For a fixed failure probability \(\delta \in (0, 1)\), our goal is to directly construct a prediction region defined by a constant \(C\), such that
% \[
% P(\rho^\phi(\hat{x}, \tau_0) - \rho^\phi(X, \tau_0) \leq C) \geq 1 - \delta. \tag{3}\label{eq:3}
% \]
%[Rewrite on Oct9] Here, \(\rho^\phi(\hat{x}, \tau_0)\) denotes the predicted robust semantics for the specification \(\phi\), which can be calculated at time \(t\) based on the observations \(x_{\text{obs}}\) and the predictions \(\hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t}\). If equation \eqref{eq:3} holds, then \(\rho^\phi(\hat{x}, \tau_0) > C\) becomes a sufficient condition for \(P(\rho^\phi(X, \tau_0) > 0) \geq 1 - \delta\) to hold. 


% [Original Text, Already Rewritten]which is the concatenation of the current observations \(x_{\text{obs}}\) and the predictions of future states \(\hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t}\). For an a priori fixed failure probability \(\delta \in (0, 1)\), our goal is to directly construct a prediction region defined by a constant \(C\) so that
% \[
% P(\rho^\phi(\hat{x}, \tau_0) - \rho^\phi(X, \tau_0) \leq C) \geq 1 - \delta. \tag{3}\label{eq:3}
% \]
% [Original Text, Already Rewritten]Note that \(\rho^\phi(\hat{x}, \tau_0)\) is the predicted robust semantics for the specification \(\phi\) that we can calculate at time \(t\) based on the observations \(x_{\text{obs}}\) and the predictions \(\hat{x}_{t+1 \mid t}, \ldots, \hat{x}_{t+H \mid t}\). Now, if equation (3) holds, then we know that \(\rho^\phi(\hat{x}, \tau_0) > C\) is a sufficient condition for \(P(\rho^\phi(X, \tau_0) > 0) \geq 1 - \delta\) to hold.





%[Rewrite on Oct9] From this, we can now compute a constant \(C\) that makes equation (3) valid and use it to solve Problem 1. By applying Lemma 1 from \cite{80}, assume without loss of generality that the nonconformity scores \(R^{(i)}\) are sorted in non-decreasing order. Additionally, let us define \(R^{(|\mathcal{D}_{\text{cal}}| + 1)} := \infty\) as the \((|\mathcal{D}_{\text{cal}}| + 1)\)-th value.

%[Rewrite on Oct9]\paragraph{\textbf{Theorem 1}}
%[Rewrite on Oct9]Consider a distribution \((X_0, X_1, \ldots) \sim \mathcal{D}\), the current time \(t\), observations \(x_{\text{obs}} := (x_0, \ldots, x_t)\), a bounded STL formula \(\phi\) enabled at time \(\tau_0\), a calibration dataset \(D_{\text{cal}}\), and a failure probability \(\delta \in (0, 1)\). The prediction region defined by equation \eqref{eq:3} is valid with \(C\) as:
% \[
% C := R^{(p)} \quad \text{where} \quad p := \lceil (|D_{\text{cal}}| + 1)(1 - \delta) \rceil - 1.
% \]
% It follows that \(P((X, \tau_0) \models \phi) \geq 1 - \delta\) if \(\rho^\phi(\hat{x}, \tau_0) > C\).

% \paragraph{\textbf{Proof}}
% The nonconformity scores \(R^{(i)}\) are independent and identically distributed (i.i.d.) based on their definition and Assumption 1. By Lemma 1 in \cite{80}, we can confirm that equation (3) holds with the specific choice of \(C\) defined in equation (4). Thus, we have:
% \[
% P(\rho^\phi(X, \tau_0) \geq \rho^\phi(\hat{x}, \tau_0) - C) \geq 1 - \delta.
% \] 
% If \(\rho^\phi(\hat{x}, \tau_0) > C\), it implies:
% \[
% P(\rho^\phi(X, \tau_0) > 0) \geq 1 - \delta,
% \]
% which further implies:
% \[
% P((X, \tau_0) \models \phi) \geq 1 - \delta,
% \]
% since \(\rho^\phi(X, \tau_0) > 0\) directly implies that \((X, \tau_0) \models \phi\), as supported by \cite{32,33}.

% Additionally, it is worth noting that neither the online verification nor the offline verification (discussed in the following framework section) requires retraining the predictor when the specification \(\phi\) changes. This is different from prior work such as \cite{68,69}, since we utilize trajectory predictors to obtain state predictions \(\hat{x}_{t \mid t}\) independent of the specific formula \(\phi\).

\subsection{STL Background}
Signal Temporal Logic (STL) is a formal language used to define temporal properties for real-valued, continuous, or discrete-time signals. Consider \( x := (x_0, x_1, \ldots) \) as a discrete-time signal, which is a realization of the stochastic system \((X_0, X_1, \ldots)\). The building blocks of STL are predicates, which are functions \(\mu : \mathbb{R}^n \to \{\text{True}, \text{False}\}\). The predicate \(\mu\) is often defined through a predicate function \( h : \mathbb{R}^n \to \mathbb{R} \) such that \(\mu(x_\tau) := \text{True} \) if \( h(x_\tau) \geq 0 \) and \(\mu(x_\tau) := \text{False}\) otherwise. The syntax of STL is recursively defined as follows:
\[
\phi ::= \text{True} \mid \mu \mid \neg \phi' \mid \phi' \land \phi'' \mid \phi' U_I \phi'' \mid \phi' U_I \phi'' 
\]

Here, \(\phi'\) and \(\phi''\) are STL formulas. The Boolean operators \(\neg\) and \(\land\) encode negations ("not") and conjunctions ("and"), respectively. The until operator \(\phi' U_I \phi''\) indicates that \(\phi'\) must hold true until \(\phi''\) becomes true within the interval \(I\).


% \paragraph{\textbf{STL Satisfaction}}STL satisfaction refers to the binary evaluation of whether a given signal fulfills an STL formula. This evaluation determines if the specified conditions hold true for the signal within predefined time intervals. The outcome of STL satisfaction is a Boolean value: the signal either satisfies the formula (True) or it does not (False). For instance, for a given STL formula \(\phi\), a signal \(x\) satisfies \(\phi\) (denoted as \(x \models \phi\)) if the conditions set by \(\phi\) are met by the signal \(x\).

% \paragraph{\textbf{Robust Satisfaction}} Denoted by $\rho^\phi(x,t)$ extends the binary nature of STL satisfaction by providing a quantitative measure of how robustly a signal satisfies or violates an STL formula. Unlike the binary outcome, robust satisfaction offers a real-valued metric: positive values indicate that the signal satisfies the formula, with the magnitude reflecting the strength of satisfaction, while negative values indicate a violation, with the magnitude representing the severity of the violation. Lets say $\phi := G_{[0,T]}(x > 750)$, $\rho^\phi(x,t)$ can be defined as $x - 750$ to quantitatively measure how robust $x$ is at time $t$. 
\paragraph{\textbf{Robust Satisfaction,}} denoted by \( \rho^\phi(x,\tau) \), extends the binary evaluation of STL satisfaction by providing a quantitative measure of the degree to which a signal satisfies or violates a given STL formula. Unlike the traditional binary satisfaction, robust satisfaction produces a real-valued metric: positive values indicate that the signal satisfies the formula, with the magnitude representing the strength of satisfaction, whereas negative values denote a violation, with the magnitude reflecting the severity of the violation. For instance, given the formula \( \phi := G_{[0,T]}(x > 750) \), the robust satisfaction can be defined as \( \rho^\phi(x,\tau):= (x - 750) \), providing a quantitative assessment of how robustly the signal \( x \) satisfies the condition at time \(\tau \).

% This quantitative measure is particularly useful in scenarios involving noise and uncertainty, as it provides insight into the degree to which a system complies with or deviates from the specified conditions. 


% \section{Problem Formulation}
% \subsection{Conformal Prediction}
% \textbf{Proof: Conformal Prediction\hanwen{Maybe we do not need to prove this one?}}

% We define the \((1 - \delta)\)-th quantile of a random variable \(Z\) as:
% \[
% \text{Quantile}_{1-\delta}(Z) := \inf\{z \in \mathbb{R} \mid P(Z \leq z) \geq 1 - \delta\}.
% \]

% Next, we define the \((1 - \delta)\)-th quantile of \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\) using the random variable \(Z_0 \sim \sum_{i=0}^{K} \delta_{R^{(i)}} / (K+1)\), where \(\delta_{R^{(i)}}\) is the Dirac distribution centered at \(R^{(i)}\). Slightly abusing notation, we define the \((1 - \delta)\)-th quantile of \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\) as:
% \[
% \text{Quantile}_{1-\delta}(R^{(0)}, R^{(1)}, \dots, R^{(K)}) := \text{Quantile}_{1-\delta}(Z_0).
% \]

% Similarly, we define the \((1 - \delta)\)-th quantile of \(R^{(1)}, \dots, R^{(K)}\) and \(\infty\) as:
% \[
% \text{Quantile}_{1-\delta}(R^{(1)}, \dots, R^{(K)}, \infty) := \text{Quantile}_{1-\delta}(Z_\infty) \tag{S4}
% \]
% with \(Z_\infty \sim \left(\sum_{i=1}^{K} \delta_{R^{(i)}} + \delta_{\infty} \right) / (K+1)\).

% \textbf{Fact 1}: Based on these definitions, consider the following. If 
% \[
% R^{(0)} > \text{Quantile}_{1-\delta}(R^{(0)}, R^{(1)}, \dots, R^{(K)}) =: q,
% \]
% then we can modify \(R^{(0)}\) to any value without changing \(\text{Quantile}_{1-\delta}\\(R^{(0)}, R^{(1)}, \dots, R^{(K)})\) as long as \(R^{(0)} > q\). If \(R^{(0)} = q\), we have \(\text{Quantile}_{1-\delta}(R^{(0)}, R^{(1)}, \dots, R^{(K)}) = \text{Quantile}_{1-\delta}(M, R^{(1)}, \dots, R^{(K)})\), where \(M > q\). This shows \(\text{Quantile}_{1-\delta}(R^{(0)}, R^{(1)}, \dots, R^{(K)})\) is equivalent to \(\text{Quantile}_{1-\delta}(M, R^{(1)}, \dots, R^{(K)})\).

% \textbf{Fact 2}: Let \(z\) take one of the values from \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\) and let \(p_z\) be the order statistic corresponding to this value. Then the probability \(P(Z_0 \leq z)\) is given by \(p_z / (K+1)\). From the definition, we know that \(\text{Quantile}_{1-\delta}(Z_0)\) corresponds to the smallest \(z\) from \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\), such that \(P(Z_0 \leq z) \geq 1 - \delta\). This implies \(p_z\) is such that \(p_z / (K+1) \geq 1 - \delta\). Since we want the smallest \(p_z\), it follows that:
% \[
% p_z = \lceil (K + 1)(1 - \delta) \rceil.
% \]
% Thus, \(R^{(0)} \leq \text{Quantile}_{1-\delta}(R^{(0)}, R^{(1)}, \dots, R^{(K)})\) is equivalent to \(R^{(0)}\) being one of the smallest \(\lceil (K + 1)(1 - \delta) \rceil\) values of \(R^{(0)}, R^{(1)}, \dots,\\ R^{(K)}\).

% \textbf{Conclusion}: Combining Facts 1 and 2, we conclude that \(R^{(0)} \leq \text{Quantile}_{1-\delta}(R^{(1)}, \dots, R^{(K)}, \infty)\) is equivalent to \(R^{(0)}\) being among the \(\lceil (K + 1)(1 - \delta) \rceil\)-th smallest values of \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\). Since \(R^{(0)}, R^{(1)}, \dots, R^{(K)}\) are independent and identically distributed, the latter (and thus the former) holds with a probability of at least \(\lceil (K + 1)(1 - \delta) \rceil / (K + 1) \geq 1 - \delta\).

% \subsection{Offline Verification}
% We may need to remove this offline verification
% \paragraph{\textbf{Assumption 1.}} We have access to $K$ independent realizations $x^{(i)} = (x_0^{(i)}, x_1^{(i)}, \ldots)$ of the distribution $D$ that are collected in the dataset $D := \{x^{(1)}, \ldots, x^{(K)}\}$.

% In “offline” system verification, e.g., in statistical model checking, we are interested in calculating the probability that $(X_0, X_1, \ldots) \sim D$ satisfies the specification.

% The goal is to verify that the output of an already trained LEC satisfies a property \(\phi_{\text{out}}\) for all inputs that satisfy a property \(\phi_{\text{in}}\). Formally, we want to verify that \(\mu(u) \models \phi_{\text{out}}\) for all inputs \(u \models \phi_{\text{in}}\), or equivalently
% \[
% \forall u \in \mathbb{R}^{n_u}, u \models \phi_{\text{in}} \implies \mu(u) \models \phi_{\text{out}}. \tag{tag}
% \]

% As a concrete example, consider an input set \(C_{\text{in}} \subseteq \mathbb{R}^{n_u}\) and an output set \(C_{\text{out}} \subseteq \mathbb{R}^{n_y}\) for which we want to verify that \(\mu(C_{\text{in}}) \subseteq C_{\text{out}}\) with \(\mu(C_{\text{in}}) := \{ y \in \mathbb{R}^{n_y} \mid \exists u \in C_{\text{in}}, \mu(u) = y \}\).

% In what follows, we apply conformal prediction to dealing with uncertainty. We will obtain practical algorithms that can compute input-output properties in real-time and with high confidence. In doing so, we give up on soundness of our verification algorithms and instead obtain probabilistically sound verification algorithms. A probabilistically sound verification algorithm for (14) provides a positive answer only if equation (14) is true with a probability no less than \(1 - \delta\).


% We are thus interested in a probability no less than \(1 - \delta\). Specifically,
% \[
% u \sim \mathcal{D}_{\phi_{\text{in}}} \implies \text{Prob}(\mu(u) \models \phi_{\text{out}}) \geq 1 - \delta \tag{tag}
% \]
% where \(\mathcal{D}_{\phi_{\text{in}}}\) is a distribution with support over the input set \(C_{\text{in}} := \{ u \in \mathbb{R}^{n_u} \mid u \models \phi_{\text{in}} \}\). Indeed, not all verification problems are deterministic and can be expressed in the form of (14), e.g., in image classification or state estimation where stochasticity has to be taken into account, and one has to instead formulate the problem in the form of (tag).


==> sections/cp-guided.tex <==
% \section{{\cp}-Guided Actual Latency Upper Bound Query Optimization}
\section{{\cp}-Guided Query Optimization}

In the previous section, we introduced {\cp} to enhance the analysis of Query Optimization procedures and detect violations during runtime verification to enable a complete re-generation at the query level. In this section, we utilize the upper bound for the actual latency with the confidence from the {\cp} model (Equation~\ref{4.3-2}) to heuristically guide the query plan generation.

\subsection{Overview}

The classical white-box {\lqo}s, such as Balsa~\cite{balsa}, employ machine learning models to predict costs $\hat{c}$ for potential sub-plans. These models are trained to approximate the actual latency $t$ with $\hat{c}$, and then select the sub-plan with the minimum $\hat{c}$ for each operator to construct the complete plan. Their goal is to find the optimal plan heuristically by sorting and selecting sub-plans solely based on minimizing the predicted cost $\hat{c}$. In contrast, our algorithm utilizes a {\cp}-guaranteed actual latency upper bound $U_{t} = \hat{c}_{\tau}^{(j)} + C$ as the guiding metric, which follows $P(t_{\tau}^{(j)} \leq U_{t}) \geq 1 - \delta$ (right inequality in Equation~\ref{4.3-2}). Minimizing this reliable actual latency upper bound at each step is our heuristic, aiming to construct a latency-optimized query plan. The detailed algorithm is presented in Alg.~\ref{alg:cp-guided}.


The following algorithm details how our {\cp}-Guaranteed method constructs a query plan using beam search. Beam Search is a heuristic search algorithm that maintains the top \( \text{beam\_size} \) candidate sequences at each round to efficiently approximate the optimal solution in large search spaces. The beam is essentially a priority queue. In our algorithm, a state in the beam includes a list of partial plans, which represents the current query plan searching status. If the state contains only one partial plan, it indicates that all relations have been connected, resulting in a complete plan. The algorithm continues until it identifies $n$ complete plans and then selects the top-ranked plan.



% \begin{algorithm}[hbtp]
% \caption{{\cp}-Guided Actual Latency Upper Bound {\lqo}}
% \label{alg:cp-guided}
% \begin{algorithmic}[1]
% \REQUIRE Learned Cost Predictor ${\texttt{LCP}}$, Substructure upper bound on the latency-cost non-conformity score $\{C_{\text{sub1}}, C_{\text{sub2}}, \dots\}$, Number of sorted candidates kept after each round ${\texttt{beam\_size}}$, Finish searching until number of complete plans $\texttt{n}$
% \ENSURE Top-ranked Plan $\texttt{final\_plan}$
% \STATE $\texttt{beam} \gets [\{start\_state\}]$ \Comment{Initialize the searching beam}
% \STATE $\texttt{complete\_plans} \gets []$ 
% \WHILE{$\texttt{len(complete\_plans)} < \texttt{n}$ \textbf{and} $\texttt{beam}$ is not empty}
%     \STATE $(\texttt{state\_cost}, \texttt{state}) \gets \texttt{beam.pop()}$
%     \IF{$\texttt{state}$ is a complete plan}
%         \STATE $\texttt{complete\_plans.add(state)}$
%         \STATE \textbf{continue}
%     \ENDIF
%     \STATE $(\texttt{new\_costs}, \texttt{potential\_plans}) \gets \texttt{explore(state)}$
%     \FOR{\textbf{each} pair \textbf{in} $(\texttt{new\_costs}, \texttt{potential\_plans})$}
%     \STATE Add pair to $\texttt{beam}$
%     \ENDFOR

%     \STATE Sort $\texttt{beam}$ by {\cp}'s actual upper bound ascending\textsuperscript{\textbf{1}}
%     \STATE $\texttt{beam} \gets \texttt{beam[:beam\_size]}$ \COMMENT{Shorten beam to beam\_size}
% \ENDWHILE
% \STATE Sort $\texttt{complete\_plans}$ by {\cp}'s actual upperbound ascending\textsuperscript{\textbf{1}}

% \STATE Select the $\texttt{complete\_plans[0]}$
% \RETURN $\texttt{final\_plan}$

% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[hbtp]
\caption{{\cp}-Guided Actual Latency Upper Bound QO}
\label{alg:cp-guided}
\begin{algorithmic}[1]
\Require Learned Cost Predictor \texttt{LCP}, Pattern upper bound on the latency-cost non-conformity score $\{C_{\text{pat1}}, C_{\text{pat2}}, \dots\}$, Number of sorted candidates kept after each round \texttt{beam\_size}, Finish searching until number of complete plans \texttt{n}
\Ensure Top-ranked Plan \texttt{final\_plan}
\State \texttt{beam} $\gets$ [\{\texttt{start\_state}\}] \Comment{Initialize the searching beam}
\State \texttt{complete\_plans} $\gets$ [] 
\While{\texttt{len(complete\_plans)} $<$ \texttt{n} \textbf{and} \texttt{beam} is not empty}
    \State (\texttt{state\_cost}, \texttt{state}) $\gets$ \texttt{beam.pop()}
    \If{\texttt{state} is a complete plan}
        \State \texttt{complete\_plans.add(state)}
        \State \textbf{continue}
    \EndIf
    \State (\texttt{new\_costs}, \texttt{potential\_plans})$\gets$\texttt{explore(LCP, state)}
    \ForAll{pair in (\texttt{new\_costs}, \texttt{potential\_plans})}
        \State Add pair to \texttt{beam}
    \EndFor
    \State Sort \texttt{beam} by {\cp}'s actual upper bound ascending\textsuperscript{\textbf{1}}
    \State \texttt{beam} $\gets$ \texttt{beam[:beam\_size]} \Comment{Shrink beam to beam\_size}
\EndWhile
\State Sort \texttt{complete\_plans} by {\cp}'s actual upper bound ascending\textsuperscript{\textbf{1}}
\State \texttt{final\_plan} $\gets$ \texttt{complete\_plans[0]}\Comment{Top-ranked plan}\\ 
\Return \texttt{final\_plan}
\end{algorithmic}
\noindent\footnotesize{[\textbf{1}] By using Alg.~\ref{Algorithm:Extract-Substructure} and Alg.~\ref{Algorithm:CP-Upperbound} and $\{C_{\text{sub1}}, C_{\text{sub2}}, \dots\}$.} 
\end{algorithm}



To start the beam search, we initialize the beam with one starting state. This \texttt{start\_state} contains separated initial partial plans, each representing one type of scan best for each relation. The size of \texttt{start\_state} equals the number of relations in the query. We also initialize an empty set to store the discovered \texttt{complete\_plans} (lines \textit{1-2}). At each iteration in the while loop, we retrieve the best options (\texttt{state\_cost}, \texttt{state}) from the beam (lines \textit{3-4}) and check if the \texttt{state} constitutes a complete plan. If it does, we add it to the set of complete plans (lines \textit{5-8}). If not, we continue the search from the current state by calling the $explore()$ function. This function iterates to fetch all potential plans by enumerating the next feasible operator from the operator selection list, introducing the partial plans in the \texttt{state} as its left or right child. It then calls the Learned Cost Predictor (\texttt{LCP}) to infer the corresponding cost for each plan, returning the related (\texttt{new\_costs}, \texttt{potential\_plans}) pair (line \textit{9}). Then, we append these newly found candidates in the beam (lines \textit{10-12}).

\begin{algorithm}[h]
\caption{Extract Pattern}
\label{Algorithm:Extract-Substructure}
\begin{algorithmic}[1]
\Function{ExtractPattern}{\texttt{state}}
% \Require State \texttt{state}
% \Ensure Substructure as a formatted string
\State \texttt{plan} $\gets$ \texttt{state} \Comment{Fetch the latest generated partial plan.}
\State \texttt{parent} $\gets$ \texttt{plan.operator}
\If{\texttt{plan.children} is empty}
    \State \Return \texttt{None} \Comment{pattern shall include children.}
\EndIf
\State \texttt{left\_child} $\gets$ \texttt{plan.children[0].operator}
\State \texttt{right\_child} $\gets$ \texttt{plan.children[1].operator}
\State \Return \texttt{(\texttt{parent},\texttt{left\_child},\texttt{right\_child})}
\EndFunction
\end{algorithmic}
\end{algorithm}

To sort the beam by the {\cp}-guided actual latency upper bound (line \textit{13}), we first use Alg.~\ref{Algorithm:Extract-Substructure} to extract the current pattern, and then use Alg.~\ref{Algorithm:CP-Upperbound} to calculate the latency upper bound. In Alg.~\ref{Algorithm:Extract-Substructure}, we begin by fetching the latest generated partial plan, enabling our {\cp} to operate on top of it and provide the latest guarantee. We first extract the parent operator. Then, we check if the current partial plan has children, as each pattern is a two-layer structure. If there are no children, we return \texttt{None}; otherwise, we return the constructed pattern. Alg.~\ref{Algorithm:CP-Upperbound} details the construction of the upper bound $U_{c}$ for a given pattern. According to Lemma 1, once a sufficient number of calibration data points (exceeding $K=\frac{1-\delta}{\delta}$) is gathered for the specific pattern, $C_{\text{pat}}$ is considered valid. Our algorithm accounts for cases where patterns may arise from combinations lacking trustworthy $C_{\text{pat}}$ values. We first check whether the detected pattern exists in \texttt{cp\_hashmap}, which contains all valid \{\text{pat}: $C_{\text{pat}}$\} pairs. If found, we pick the corresponding $C_{\text{pat}}$; otherwise, we assign $C_{\text{pat}}$ the maximum value among the available $C_{\text{pat}}$ (correctness will be discussed in Section~\ref{sec:alg-analysis}). Finally, we add the predicted cost and this \texttt{latency\_cost\_upperbound} to fetch the {\cp}-guaranteed actual latency upper bound.
\begin{algorithm}[hbtp]
\caption{Calculate {\cp} Guaranteed Latency Upper Bound}

\label{Algorithm:CP-Upperbound}
\begin{algorithmic}[1]
\Require Pattern hashmap \texttt{cp\_hashmap} = \{\text{pat}: $C_{\text{pat}}$\}
\Function{CPLatencyUpperBound}{\texttt{cost}, \texttt{state}, \texttt{cp\_hashmap}}
\State \texttt{pattern} $\gets$ \texttt{extract\_pattern(state)} 
\If{\texttt{pattern} $\in$ \texttt{cp\_hashmap}}
    \State \texttt{latency\_cost\_upperbound}$\gets $\texttt{cp\_hashmap[pattern]}
\Else \Comment{Pattern not present in {\cp} hashmap}
    \State \texttt{latency\_cost\_upperbound} $\gets \max(C_{\text{pat}}) $
\EndIf
\State \Return \texttt{cost} + \texttt{latency\_cost\_upperbound}
\EndFunction
\end{algorithmic}
\end{algorithm}

Then, we limit the beam to a maximum of \texttt{beam\_size} elements (line 14). After identifying $n$ complete plans, we use a sorting method similar to that in line 13 to rank these complete plans. One important detail is that, during the loop, we need to find the latest generated partial plan from multiple partial plans in each state; however, in the final complete plan selection, each state contains only one complete plan. Finally, we return the top-ranked \texttt{final\_plan} (lines 16-18).

% \begin{algorithm}[hbtp]
% \caption{Calculate {\cp} Guaranteed Upper Bound}
% \label{Algorithm:CP-Upperbound}
% \begin{algorithmic}[1]
% \Require Cost \texttt{cost}, State \texttt{state}, CP Values \texttt{cp\_hashmap}
% \State \Comment{Extract substructure based on state}
% \State \texttt{substructure} $\gets$ \texttt{extract\_substructure(state)}
% \If{\texttt{substructure} $\in$ \texttt{cp\_hashmap}}
%     \State \texttt{quantile\_c} $\gets$ \texttt{cp\_hashmap[substructure]}
% \Else
%     \State \texttt{quantile\_c} $\gets$ the largest quantile \Comment{Substructure not present in {\cp} hashmap}
% \EndIf
% \State \Return \texttt{cost} + \texttt{quantile\_c}
% \end{algorithmic}
% \end{algorithm}




\subsection{Algorithm Analysis}\label{sec:alg-analysis}
We formulate our method as greedy algorithms; we will show its correctness, effectiveness, and complexity in this section.


% \noindent\textbf{Correctness.} 
\subsubsection{Correctness} We prove the correctness by discussing the following three conditions. 

\begin{enumerate}
    \item All patterns are in \texttt{cp\_hashmap}. If all patterns have corresponding valid $C_{\text{pat}}$ values, the algorithm directly calculates the actual latency upper bound by summing the current predicted cost and the latency-cost upper bound provided by the {\cp} model. These values are then used in the subsequent sorting.
    \item No patterns are in \texttt{cp\_hashmap}. In this case, a fixed value is added to all predicted costs. Since the same arithmetic logic applies to each value, this adjustment does not affect the original ordering. The output orders are based on the predicted costs. 
    \item Partial patterns are in \texttt{cp\_hashmap}. In this scenario, valid patterns are added to their corresponding latency-cost upper bound, while the remaining patterns are added a fixed value equal to the largest latency-cost upper bound. This approach prioritizes valid patterns with {\cp} guarantees while still allowing for the possibility of extending from other patterns. 
\end{enumerate}


% \noindent\textbf{Effectiveness.} 
\subsubsection{Effectiveness}Our algorithm enhances traditional cost-based methods by not merely selecting the minimum cost with the hope of achieving minimal latency during actual execution. Instead, our approach sets a {\cp}-guaranteed latency upper bound as the target, which serves as a more direct heuristic. At each step, we extend the current partial plan by adding one more operator. Since the final complete plan consists of a finite number of operators, the algorithm is guaranteed to terminate. The output is a complete plan guided by the {\cp}-based heuristic.

% \noindent\textbf{Complexity.} 
\subsubsection{Complexity}This algorithm retains the beam search logic, with the only addition being the calculation of the {\cp}-guided actual latency upper bound. The upper bound calculation in Alg.~\ref{Algorithm:CP-Upperbound} operates in constant time, i.e., $O(1)$. Additionally, all computations are performed in-place, requiring no extra storage space. Therefore, our {\cp}-upper bound guided algorithm maintains the same time and space complexity as the baseline beam search method.


==> sections/formulation.tex <==
\section{Problem Formulation}
% 
In a database system, query plans are constructed operator by operator within the query optimizer. This process is analogous to robot movement: robots make decisions based on model predictions and then generate a trajectory. Similarly, in our database context, sub-plans are selected based on predictions from an analytical component. These sub-plans are then assembled into a complete query plan. The generated query plan is then executed on actual data and used to fetch results. These steps in the planning and execution stages are tightly coupled, corresponding one-to-one. 
\subsection{Conformal Prediction}
In an ML-based Query Optimizer, each step of constructing the sub-plan is guided by the ML model's predicted cost. During the execution phase, we measure the corresponding actual runtime for each step. Our research focuses on how to gain insights into these plans' quality before executing them by using the predicted costs. Specifically, we study how the actual time fluctuates relative to the predicted cost. We denote the predicted cost as $\hat{C}$ and the actual time as $T$. Then, we take the nonconformity score \(R := \lVert T-\hat{C} \rVert\) or \(R := (T-\hat{C})\). For clarity, we will use \(R:=\lVert T - \hat{C} \rVert \) in the following discussion. We take each step \(\tau\) in the query plan construction process \(j\), then we can construct the database context nonconformity score as:
\[
R^{(i)} := \lVert t_{\tau}^{(j)} - \hat{c}_{\tau}^{(j)} \rVert .\tag{2}\label{3.1-1}
\]

With this formula, we can construct nonconformity sequences \( R^{(i)}:= \{R^{0}, R^{1}, \dots, R^{K}\} \), and then we derive a probabilistic prediction region with confidence as described in Equation (\ref{2.2-1}). In our context, \(C\) measures the difference between the predicted cost and actual runtime. The construction works as follows: For a given failure probability \(\delta \in (0, 1)\), we compute the upper bound \(C : \mathbb{R}^K \to \mathbb{R}\) as:
\[
C := \text{Quantile}_{1-\delta}(R^{(1)}, \dots, R^{(K)}, \infty), 
\tag{3}\label{3.1-2}
\]
which represents the \((1 - \delta)\)-th quantile over the empirical distribution of the values \(R^{(1)}, \dots, R^{(K)}\), with \(\infty\) included as a correction to ensure finite sample guarantees. Without loss of generality, we assume that \(R^{(1)}, \dots, R^{(K)}\) are sorted in non-decreasing order, which can easily be achieved by re-ordering the values. We then set \(R^{(K+1)} := \infty\). Applying this with the \( R^{(i)} \) sequences, we can get the upper bound \( C\):
\[
C := R^{(p)} \quad \text{where} \quad p := \lceil (|D_{\text{cal}}| + 1)(1 - \delta) \rceil - 1. \tag{4}\label{3.1-3}
\]
where \(\lceil \cdot \rceil\) denoting the ceiling function, \(C\) is actually the \(p\)-th smallest nonconformity score.

% \textbf{Lemma 1 (Marginal Coverage)\hanwen{Maybe we do not need to prove this one? This is just to prove that C can be used for R0}}.
% Let \(R^{(0)}, \dots, R^{(K)}\) be \(K + 1\) independent and identically distributed (i.i.d.) random variables. Then, the probabilistic prediction region in equation (xx) is valid based on the selection of \(C\) as defined in equation (xx). We provide the proof below. The proof is largely inspired by []\cite{x}. 

% Then with the previous Lamma 1 and related proof, we can get the marginal coverage guarantee from conformal prediction on the database query optimizer:

\textbf{How much calibration data is required?} Fetching enough calibration data for constructing a valid conformal prediction model is important. We get this boundary from the computation process for the upper bound \(C\). Based on equations (2-3), we fetch \(p^{th}\) value from the non-decreasing series \((R^{(1)}, \dots, R^{(K)}, \infty)\). If \(\lceil (K+1)(1-\delta) \rceil > K\), the upper bound \(C\) becomes trivial and uninformative, yielding \(C = \infty\). To ensure that the upper bound is nontrivial, we need the condition \(\lceil (K+1)(1-\delta) \rceil \leq K\). From this, We get a lower bound on the amount of data required to compute a meaningful upper bound \(C\):
\[
K \geq \frac{1 - \delta}{\delta}
\]

\textbf{Marginal Coverage Guarantees.} We would like to highlight that the guarantee in the equation is marginal, referring to the randomness across both the test and calibration data points \(R^{(0)}, R^{(1)},\\ \dots, R^{(K)}\), rather than conditional on the specific values of the calibration set \(R^{(1)}, \dots, R^{(K)}\). In other words, \(\text{Prob}(\cdot)\) reflects the randomness arising from the draw over all random variables. 

Based on the previous discussion, we conclude the core formula we use in our framework as follows:
\[
P(\lVert t^{(i)} - \hat{c}^{(i)} \rVert \leq C) \geq 1 - \delta. \tag{5}\label{eq:5}
\]
where \(i\) means the data point index in our data series. We construct \(C\) based on the calibration set and then apply this \(C\) and \(\delta\) to other data points to provide the same guarantees. In our framework, this conformal prediction formula offers us guarantees with confidence.

\subsection{Runtime Verification}
With conformal prediction, we can retrieve the upper bound \(C\) to define a high-confidence region that quantifies the difference between the predicted cost and the actual runtime. We aim to extend conformal prediction further by assessing the query plan quality and predicting poor plan generations (violations) during the runtime.

Suppose \(\mathcal{D}\) be a distribution which describes learned query optimizer behaviors. Let \(X := (X_0, X_1, \dots) \sim \mathcal{D}\) represent a random query plan construction process, where \(X_{\tau}\) denotes the state of generated query plan of \(\tau\) operations. We use lowercase letters \(x_{\tau}\) for realizations of the random variable \(X_{\tau}\). Then we get a realization of \(X\) as \((x_0, x_1, \ldots)\). Assume that we have observed \(x_{\text{obs}} := (x_0, \ldots, x_\tau)\), meaning the target query plan has constructed \(\tau\) operations, while the future construction \(x_{\text{un}} := (x_{\tau+1}, x_{\tau+2}, \ldots)\) remain unknown. Thus, the entire query plan construction process can be expressed as \(X:= (X_{\text{obs}}, X_{\text{un}})\) without dependent on the current operation \(\tau\). 

In the following discussion, we aim to determine the probability that \((X) \models \phi\), where \( \phi \) is an STL predicate that takes the predicted cost or actual runtime of query optimizers as input. For mainstream query optimizers, the future predictions are based on decisions that have already been made, and each time, they can only predict one operation further. Therefore, we can define the predicted trajectory as follows:
\[
\hat{x} := (x_{\text{obs}}, \hat{x}_{\tau+1 \mid \tau}) \label{3.2-1}\tag{5}
\]
which represents the concatenation of the current observations \(x_{\text{obs}}\) and the predictions of next operation \(\hat{x}_{\tau+1 \mid \tau}\). Given a fixed failure probability \(\delta \in (0, 1)\), our goal is to construct a prediction region defined by a constant \(C\), such that   
\[
P(\rho^\phi(\hat{x}) - \rho^\phi(X) \leq C) \geq 1 - \delta. \tag{6}\label{3.2-2}
\]
Here, \(\phi\) is the specification designed to verify query plans' quality, \(\rho^\phi(X)\) indicates how robustly the specification \(\phi\) is satisfied and violated with our query plan. \(\rho^\phi(\hat{x})\) denote the robust semantics from the prediction, which can be calculated at operation \(\tau\) based on the observations \(x_{\text{obs}}\) and the prediction \(\hat{x}_{\tau+1 \mid \tau}\). For each calibration operation \(x^{(i)} \in \mathcal{D}_{\text{cal}}\), we compute the nonconformity score as:
\[
R^{(i)} := \rho^\phi(\hat{x}^{(i)}) - \rho^\phi(x^{(i)}),\label{3.2-3}\tag{7}
\]
where \(\hat{x}^{(i)} := (x_{\text{obs}}^{(i)}, \hat{x}_{\tau+1 \mid \tau}^{(i)})\). We then calculate the upper bound \(C\) based on the previous formula (\ref{3.1-3}). The next step is to reformulate from formula (\ref{3.2-2}), resulting in:

% A positive nonconformity score \(R^{(i)}\) indicates that our predictions are too optimistic, i.e., that the predicted robust semantics \(\rho^\phi(\hat{x}^{(i)}, \tau_0)\) exceeds the actual robust semantics \(\rho^\phi(x^{(i)}, \tau_0)\) computed using the true calibration trajectory \(x^{(i)}\). On the other hand, a negative \(R^{(i)}\) implies that our predictions are too conservative. \hanwen{Will align with the previous conformal prediction} 
\[
P(\rho^\phi(X) \geq \rho^\phi(\hat{x}) - C) \geq 1 - \delta.\label{3.2-4}\tag{8}
\]
If \(\rho^\phi(\hat{x}) > C\), it implies:
\[
P(\rho^\phi(X) > 0) \geq 1 - \delta,\label{3.2-5}\tag{9}
\]
which further implies:
\[
P(X \models \phi) \geq 1 - \delta,\label{3.2-6}\tag{10}
\]
since \(\rho^\phi(X) > 0\) directly implies that \(X \models \phi\).

Additionally, it is worth noting that neither the guarantee method nor the runtime verification (which will be discussed more in the following framework section) requires retraining the predictor when the specification \(\phi\) changes. This is different from prior work such as \cite{68,69}, since we utilize predictors to obtain state predictions \(\hat{x}_{\tau+1 \mid \tau}\) independent of the specific formula \(\phi\).

==> sections/framework.tex <==
\section{{\cp} for {\lqo} General Framework}\label{sec:framework}

Once the {\lqo} finishes training, we construct the {\cp} model using the calibration query workload $\mathcal{Q}^{Cal}$. This {\cp} model can then seamlessly integrate into the normal {\lqo} workflow without modifying any plan-generation logic or the learned query model. Based on different integration use cases, we propose the Latency Guarantee framework and the Runtime Verification framework. These two frameworks are illustrated in Fig.~\ref{fig:framework}.

\begin{figure*}[htbp]
    \begin{subfigure}[t]{0.5\textwidth} 
        \hspace{-20pt}
        \includegraphics[height=2.8cm]{figures/framework/Latency Guarantees.pdf}
        \caption{Latency Guarantees} 
        \label{fig:latency-guarantee-framework}
    \end{subfigure}%
    \hspace*{\fill}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[height=2.8cm]{figures/framework/Runtime Verification.pdf}
        \caption{Runtime Verification} 
        \label{fig:runtime-verification-framework}
    \end{subfigure}%
    \hspace*{\fill}
    \caption{Conformal Prediction for Learned Query Optimization General Framework}
    \label{fig:framework}
\end{figure*}

\subsection{Overview}
\noindent\textbf{{\cp} Construction:} 
Given a trained {\lqo}, we observe its behavior. For each calibration operation \(x^{(i)} \in \mathcal{Q}^{\text{cal}}\), we collect the predicted cost \(\hat{c}^{(i)}\) during the {\lqo}'s plan construction and the actual latency \(t^{(i)}\) from the query execution. We use a formula similar to equation~\ref{3.1-1} to compute the non-conformity scores \(\mathbf{R}^{(i)}\). To demonstrate generalization, we define \(R^{(i)} := f(t^{(i)} - \hat{c}^{(i)})\) in our algorithm. The entire construction process is summarized in Alg.~\ref{Algorithm:Quantile-Calculate}.

% \begin{algorithm}[hbtp]
% \caption{Conformal Prediction Construction}
% \label{Algorithm:Quantile-Calculate}
% \begin{algorithmic}[1]
% \REQUIRE Prediction $\mathbf{\hat{C}}$, Ground truth $\mathbf{T}$, Failure rate $\delta = 0.1$\\
% Size$(\hat{C}, T) = K; \, K > \frac{1-\delta}{\delta}$
% \ENSURE Quantile of the non-conformity scores
% \STATE Compute the non-conformity scores $\mathbf{R}$, where $R^{(i)} = f(\hat{c}^{(i)} - t^{(i)})$ for each $\hat{c}^{(i)}$ from $\mathbf{\hat{C}}$ and $t^{(i)}$ from $\mathbf{T}$
% \STATE Let $n \gets \text{length of sorted } \mathbf{R}$
% \STATE Insert $\infty$ into the non-conformity scores: $\mathbf{R} \gets \mathbf{R} \cup \{\infty\}$
% \STATE Sort the non-conformity scores $\mathbf{R}$ in non-decreasing order
% \STATE Compute the target index $p = \lceil (n + 1)(1 - \delta) \rceil - 1$
% \STATE Retrieve the quantile $C \gets \mathbf{R}^{(p)}$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[hbtp]
\caption{Conformal Prediction Construction}
\label{Algorithm:Quantile-Calculate}
\begin{algorithmic}[1]
\Require Prediction $\mathbf{\hat{C}}$, Ground truth $\mathbf{T}$, Failure rate $\delta = 0.1$
\State\textbf{Assume} Size$(\hat{C}, T) = K$ with $K > \frac{1 - \delta}{\delta}$
\Ensure Quantile of the non-conformity scores
\State Compute the non-conformity scores $\mathbf{R}$, where $R^{(i)} = f(\hat{c}^{(i)} - t^{(i)})$ for each $\hat{c}^{(i)}$ from $\mathbf{\hat{C}}$ and $t^{(i)}$ from $\mathbf{T}$
\State Let $n \gets$ length of sorted $\mathbf{R}$
\State Insert $\infty$ into the non-conformity scores: $\mathbf{R} \gets \mathbf{R} \cup \{\infty\}$
\State Sort the non-conformity scores $\mathbf{R}$ in non-decreasing order
\State Compute the target index $p = \lceil (n + 1)(1 - \delta) \rceil - 1$
\State Retrieve the quantile $C \gets \mathbf{R}^{(p)}$
\end{algorithmic}
\end{algorithm}





\noindent\textbf{Latency Guarantees:} When a user submits a query, the trained {\lqo} generates a query plan. An uncertainty probability \(\delta\) is used to construct the {\cp} model. The query plan is then fed into the constructed {\cp} model. Based on the formulation in equation~\ref{4.3-2}, our {\cp}-based latency guarantees framework estimates the guaranteed ranges for the actual latency before executing the plan. Fig.~\ref{fig:latency-guarantee-framework} illustrates this process and outputs the guaranteed range for each level. This approach provides insights into the actual latency, even during query planning.

\noindent\textbf{Runtime Verification:} Fig.~\ref{fig:runtime-verification-framework} shows that the {\cp} model works in closer collaboration with the {\lqo}. They can be considered as a unified entity that processes user-submitted queries and outputs a verified query plan. This query plan satisfies the input constraint \(\phi\) under the uncertainty \(\delta\). The verified plan is then submitted to the execution engine for safer execution. 


\noindent\textbf{Violation Handling:} If the plan generated by the {\lqo} is found to be poor or suboptimal based on our constraint \(\phi\), our framework identifies it as a violation. The framework then discards the suboptimal plan and regenerates a new one (check Section~\ref{sec:violation}). We also have the option to regenerate at the sub-plan level. A poorly optimized plan can take much longer to execute, sometimes lasting minutes in large databases, compared to a trusted plan. In contrast, the regeneration time is in milliseconds, which is considered acceptable. This ensures that the query engine only executes query plans from the {\lqo} that have been verified by {\cp}.


% In this section, we begin by presenting the overall architecture in Sec.~\ref{sec:overall-architecture}, which demonstrates how conformal prediction verification can be easily integrated into the learned query optimizer workflow. Next, we introduce conformal prediction construction in Sec.~\ref{sec:cp-construction} and conformal prediction guarantee in Sec.~\ref{sec:cp-guarantee}. We introduce several conformal prediction verification methods with two levels of granularity in Sec.~\ref{sec:multi-granualrity}. Then, We present our runtime verification in Sec.~\ref{sec:runtime-verification}. 

% \TODO{Hanwen is updating this section}In this section, we first present the overall architecture in Sec.~\ref{sec:overall-architecture}, which illustrates how conformal prediction can be seamlessly incorporated into the workflow of learned query optimizers. Following this, we describe the process of constructing the conformal prediction model in Sec.~\ref{sec:cp-construction}. Next, in Sec.~\ref{sec:cp-guarantee}, we discuss the guarantees offered by conformal prediction. Sec.~\ref{sec:multi-granualrity} introduces multiple methods for verification, each providing different levels of granularity. Lastly, we explain the runtime verification mechanism in Sec.~\ref{sec:runtime-verification}.


% \subsection{Overall Architecture}\label{sec:overall-architecture}
% We propose the CP4LQO general framework. The core architecture is illustrated in Fig.~\ref{fig:CP4LQO-framework}. The primary objective of our framework is to verify learned query optimizers, ensuring that the generated query plans are not excessively suboptimal when submitted for execution in the query engine. The conformal prediction approach provides our assessments rigorous confidence $(1 - \delta)$.

% We separate our {\cp}-based framework into three parts. First we construct one  

% Fig.~\ref{large-framework-graph} shows the latency guarantee workflow and runtime verification workflow. In Fig.~\ref{guarantee-framework-graph}, the user submits queries and the {\lqo} based on the data distribution in the database to generate a query plan. That query plan 

% The left part of Fig.\ref{fig:CP4LQO-framework} depicts a typical query optimizer workflow. The learned query optimizers are trained and fixed, generating query plans based on the input query and the actual data distribution in the database. In our framework, we apply conformal prediction to provide guarantees and verification for this query generation process. We construct the conformal prediction model by examining the predicted cost during the query generation stage and the actual runtime during execution in the calibration set. The constructed conformal prediction tool outputs a prediction region that quantifies the difference between the predicted cost and the actual runtime with a given confidence. This prediction region is then applied to the predicted cost to provide insights into the actual runtime, which can reflect the quality of the query plan.

% Given the different mechanisms of query optimizers, we offer two types of guarantees: \toprof{these words do not make much sense, we need to check with Prof.} injected and subsequent conformal prediction. If the learned query optimizer's plan generation process is transparent to the system, allowing us to observe the prediction and decision-making processes in real-time, conformal prediction can be used during the plan construction to provide guarantees. If the query optimizer is treated as a black-box model, meaning no intermediate sub-plans are accessible for examination, we integrate conformal prediction around the constructed plan. This method takes the output of the learned query optimizer and then performs conformal prediction. \toprof{Shall we re-organise this? Because we will describe details later.} Our framework further provides two types of granularity for conformal prediction guarantees: unified guarantee and sub-structural guarantee.

% Besides guarantees, we also offer runtime verification, which is based on formal verification to detect and prevent the execution of suboptimal query plans in real-time. After verification, if a violation is detected, which is indicated by a red lightning icon in Fig.~\ref{fig:CP4LQO-framework}, it implies that according to our conformal prediction framework, the current query plan (or sub-plan) may break the specification we set within the given probability of \((1-\delta)\). When this situation arises (as shown by the dashed lines in the figure), the verification module detects such violations and can respond by either discarding the current plan and generating a new one or reverting to the default query planner provided by the underlying engine. If a new plan is generated, it undergoes re-validation, and upon successful validation, it is passed to the execution engine for actual execution. Given the computational efficiency of the conformal prediction module, this process introduces minimal delay to the overall system.



\subsection{Multi-Granularity {\cp}}\label{sec:multi-granularity-cp}
As discussed in Section~\ref{sec:background_lqo}, we categorize {\lqo}s as either white-box or black-box based on the transparency of their query plan construction to the system. Our framework designs different granularities for each of these categories.

\subsubsection{Whole-Plan {\cp}}\label{sec:whole-plan-cp} This approach is designed for black-box {\lqo}s, which output a query plan without providing intermediate analysis details. In this case, we perform whole-plan level {\cp} to guarantee and verify the results. For each query \(Q^{(i)} \in Q^{\text{Cal}}\), we measure the overall plan performance using either the output from the {\lqo} or with assistance from a mature query optimizer, such as PostgreSQL, to obtain the predicted cost \(\hat{c}^{(i)}\). Using the actual latency \(t^{(i)}\), we can then compute the non-conformity scores \(\mathbf{R}^{(i)}\) and construct the complete {\cp} model.

\subsubsection{Unified (Sub-Plan) {\cp}}\label{sec:unified-cp}

\begin{figure}[htbp]
\centering 
\includegraphics[width=0.9\linewidth]{figures/framework/unified.pdf}
\caption{Unified Sub-Plan {\cp} Workflow.} 
\label{fig:unified-conformal-prediction}
\end{figure}

For white-box {\lqo}s, which provide transparency during query plan construction, our framework captures more granular details. The machine learning models in these {\lqo}s predict costs at each level and make decisions based on these predictions. In unified sub-plan {\cp}, our framework treats all sub-plans equally, constructing non-conformity scores based on sub-plan level predicted costs and actual latencies as follows:
\[
R^{(i)} := \lVert \hat{c}^{(\tau)}_j - t^{(\tau)}_j \rVert,
\]
where data is extracted from each query \(j\) and each intermediate level \(\tau\). In addition to constructing the {\cp} model, our framework can also apply {\cp}-based guarantees and runtime verification in a more fine-grained manner, as shown in Fig~\ref{fig:unified-conformal-prediction}.


After constructing the unified {\cp} model, we obtain the same quantile \(C\) for all levels. In our example, \(C = 10\). During the {\lqo} plan generation, we extract the predicted cost at different levels as \(\hat{c} = [60, 100, 150]\). Then, following equation~\ref{4.3-2}, we construct guaranteed ranges for each level, as shown in the right part of the figure. For runtime verification, the logic is similar: the constructed unified {\cp} model examines each level and applies the same violation detection logic.


% Using the upper bound \(C\) derived from the conformal prediction model, we can perform guarantees, as seen in equation~\ref{4.3-2}, to obtain a high-confidence range for the actual runtime. In Fig.~\ref{fig:unified-conformal-prediction}, In unified conformal prediction method, the constant $C$ is uniformly applied across all stages of the query plan. As the plan is constructed, we obtain the predicted costs at each stage (e.g., 80, 100, 150). To compute the confidence intervals, we add and subtract the value of $C$ from these predicted costs. This provides a range that estimates the actual runtime with the desired level of confidence, ensuring consistency across all levels of the query plan.



% \subsection{Conformal Prediction Guarantee[Rename]}\label{sec:cp-guarantee}


% After constructing the CP model in the calibration set, we can then integrate it into our framework. Specifically, the region for actual runtime \(t^{(i)}\) will be computed based on the predicted cost \(\hat{c}^{(i)}\) and the prediction region \(C\). Recall that our constructed conformal prediction model provides the following guarantee with confidence \(1 - \delta\):
% \[
% P(\lVert t^{(i)} - \hat{c}^{(i)} \rVert \leq C) \geq 1 - \delta. \label{4.3-1}\tag{11}
% \]
% We can easily reformulate this equation into the following form:
% \[
% P(\hat{c}^{(i)} - C \leq t^{(i)} \leq \hat{c}^{(i)} + C) \geq 1 - \delta. \label{4.3-2}\tag{12}
% \]


% \subsubsection{For White-box {\lqo}s}\label{sec:injected}
% This method is designed for the query optimizers whose planning process is transparent to our framework, which maps the second category of {\lqo} in Sec.~\ref{sec:background_lqo}. For example, Balsa\cite{balsa} generates the query plan incrementally, constructing each step based on machine learning predicted costs. We can directly integrate our conformal prediction model into the planning process for such query optimizers. This integration requires no modification to the original machine learning model or interference with the plan generation procedure. When a sub-plan is generated with a predicted cost, we apply our conformal prediction model to obtain insights into the actual execution time and the plan's quality. Since the guarantee phase only involves a simple computation like Equ.~\ref{4.3-1}, our conformal prediction model is lightweight, providing reliable guarantees without adding significant overhead.


% \subsubsection{For Black-box {\lqo}s}\label{sec:subsequent} 

% The method is designed for black-box-like learned query optimizers, which map to the third category of {\lqo} mentioned earlier. They directly generate hints or provide insights for the query optimization process. For instance, Lero compares and ranks candidate plans and then outputs the best plan. In these situations, our framework can be supported from two perspectives. If a high-level analysis is needed, we can perform conformal prediction at the SQL level to guarantee plan quality. If a detailed analysis is needed, and we do not have fine-grained predictions, we can introduce a trustworthy query planner to assist. For example, PostgreSQL can follow the {\lqo}s' hints to construct a complete query plan and obtain predicted costs for each level. We can then analyze and obtain the same conformal prediction guarantees described in the previous section.



% \subsection{Sub-plan Conformal Prediction}\label{sec:multi-granualrity}
% In the context of \textit{white-box} LQOs our framework handles sub-plans at two distinct levels of abstraction. In the first approach, referred to as \textit{Unified Conformal Prediction}, all sub-plans are considered equal, disregarding their internal structure. In the second approach, called \textit{Sub-structure Conformal Prediction}, the specific patterns within the sub-plans are analyzed, allowing for more tailored predictions based on their configurations.

% \subsubsection{Unified Conformal Prediction}
% Learned model builds the query plan incrementally, constructing
% one sub-plan at a time and predicting its associated cost. Unified Conformal Prediction is agnostic of the sub-plan internals and treats all sub-plans as equals. Sub-plan's actual runtime is also captured to calculate the non-conformity scores.
% \[
% R^{(i)} := \lVert \hat{c}^{(\tau)}_j - t^{(\tau)}_j \rVert
% \]
% where \(\hat{c}^{(\tau)}_j\) represents the predicted cost at level \(\tau\) for query \(j\), and \(t^{(\tau)}_j\) represents the corresponding actual runtime. We then proceed by utilizing the algorithm outlined earlier in Sec.~\ref{sec:problem_formulation} to systematically build the conformal prediction model. This involves applying the nonconformity scores calculated for each sub-plan and using them within the framework to derive the guaranteed prediction intervals, ensuring that the model can offer confidence intervals for the predicted costs with respect to the actual runtimes.

% \begin{figure}[htbp]
% \centering 
% \includegraphics[width=\linewidth]{figures/unified.png}
% \caption{Unified Conformal Prediction. We apply same upper bound \(C\) from the conformal prediction for all the intermediate steps. \TODO{Use more compact graph to reduce the height?}} 
% \label{fig:unified-conformal-prediction}
% \end{figure}

% Using the upper bound \(C\) derived from the conformal prediction model, we can perform guarantees, as seen in equation~\ref{4.3-2}, to obtain a high-confidence range for the actual runtime. In Fig.~\ref{fig:unified-conformal-prediction}, In unified conformal prediction method, the constant $C$ is uniformly applied across all stages of the query plan. As the plan is constructed, we obtain the predicted costs at each stage (e.g., 80, 100, 150). To compute the confidence intervals, we add and subtract the value of $C$ from these predicted costs. This provides a range that estimates the actual runtime with the desired level of confidence, ensuring consistency across all levels of the query plan.

\subsubsection{Sub-structure {\cp}}\label{sec:sub-structure-cp} In sub-structure conformal prediction, more internal details of the sub-plans are taken into consideration. We extract the structure from these sub-plans and then construct separate {\cp} models for these sub-structures. This allows for more fine-grained analysis based on {\cp}. Fig.~\ref{fig:sub-structure-conformal-prediction-example} shows two examples of sub-structures. Each sub-structure is represented by a parent operator and two child operators~\footnote{Note that the child operators and their order are important for certain operations, such as hash-join, where the roles of the left and right child operators are not interchangeable.}. This can be represented as (Parent operation, left-child operation, or right-child operation). For example, the left sub-structure in Fig.~\ref{fig:sub-structure-conformal-prediction-example} can be noted as (HJ, HJ, SS).

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/framework/sub-structure1.pdf}  
        \caption{Sub-structure: (HJ, HJ, SS)}
        \label{fig:sub-structure1}
    \end{subfigure}
    \hfill 
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/framework/sub-structure2.pdf}  
        \caption{Sub-structure: (HJ, SS, SS)}
        \label{fig:sub-structure2} 
    \end{subfigure}
    \caption{Sub-structure examples}
    \label{fig:sub-structure-conformal-prediction-example}
\end{figure}



% \begin{figure}[htbp]
% \centering 
% \includegraphics[width=\linewidth]{figures/Sub_structure/PatternExamples.png}
% \caption{Sub-structure examples} 
% \label{fig:sub-structure-conformal-prediction-example}
% \end{figure}

To construct the sub-structure {\cp}, we take the predicted cost \(\hat{c}_{\text{sub}}\) and the actual latency \(t_{\text{sub}}\) to compute the non-conformity scores \(\mathbf{R}_{\text{sub}}\) as follows:
\[
R^{(i)}_{\text{sub}} := \left\lVert \hat{c}_{\text{sub}}^{(i)} - t_{\text{sub}}^{(i)} \right\rVert,
\]
where the subscript "sub" refers to the sub-structure, for example, (HJ, SS, SS). Using these non-conformity scores $R_{\text{sub}}$, we can obtain corresponding quantiles $C_{\text{sub}}$ for the target sub-structures. During the construction of test query plans, the predicted sub-structures are identified at each level. The corresponding \(C_{\text{sub}}\) value is then applied to provide a guaranteed region based on the predicted cost.

\begin{figure}[htbp]
\centering 
\includegraphics[width=0.9\linewidth]{figures/framework/sub-structure-cp.pdf}
\caption{Sub-structural Conformal Prediction} 
\label{fig:sub-structure-conformal-prediction}
\end{figure}

% Using this series $\mathbf{R}$ and Alg(\ref{Algorithm:Quantile-Calculate}) we compute an upper bound \(C_{\text{sub}}\), which varies across different sub-structure types. Each unique sub-structure type in the calibration set yields its own \(C_{\text{sub}}\), ensuring that the prediction bounds are specific to the query plan components.

% \begin{figure}[htbp]
% \centering 
% \includegraphics[width=0.8\linewidth]{figures/Sub_structure/PatternCP.png}
% \caption{Sub-structural Conformal Prediction} 
% \label{fig:sub-structure-conformal-prediction}
% \end{figure}


Fig.~\ref{fig:sub-structure-conformal-prediction} illustrates how we perform sub-structure level {\cp} on different sub-structures. The {\lqo} constructs the query plan from bottom to top. It first constructs a Hash Join (HJ) at the first level, with the left child as a Sequential Scan (SS) and the right child also as SS. Following the previous definition, this sub-structure is denoted as (HJ, SS, SS). The {\lqo} gives a predicted cost as 60. From our corresponding sub-structure {\cp}, the quantile \(C_{\text{(HJ,SS,SS)}} = 5\), and we can generate the guaranteed range for the actual latency of the sub-structure as \([55, 65]\). Following this workflow, we construct other guaranteed ranges as \([90, 110]\) for the sub-structure (HJ, HJ, SS), and \([100, 200]\) for the sub-structure (HJ, HJ, IS). This method provides us with finer-granularity analysis and control for the {\cp} model.



\subsection{Violation Handling}\label{sec:violation}
As stated in Lemma 2, our {\cp} model approves the generated plan if \(\rho^\phi(\hat{x}) > C\), as this implies \(\text{Prob} (X \models \phi) \geq 1 - \delta\). If a violation is detected when \(\rho^\phi(\hat{x}) \leq C\), the current query plan will be discarded, and a new one will be regenerated. It is important to note that our {\cp}-based runtime verification framework can detect violations not only after constructing a complete plan but also during query plan construction for white-box {\lqo}s.

\begin{figure}[hbtp]
    \centering
    \includegraphics[width=\linewidth]{figures/framework/runtime-violation-detection.pdf}
    \caption{Runtime Violation Handling}
    \label{fig:runtime-violation-handling}
\end{figure}

Fig.~\ref{fig:runtime-violation-handling} illustrates our violation-handling process. When the {\lqo} generates a query plan, the {\cp} model performs verification during the intermediate steps. The colored icons represent the portions of the query plan that have already been generated, while the dashed boxes indicate the steps yet to be completed. If the {\cp} model detects a violation, the Reliable Query Optimizer generates a new query plan. Then, this regenerated query plan will be executed by the query engine.


% During the construction of test query plans, the predicted sub-structures are identified at each level. The appropriate \(C_{\text{sub}}\) value is then applied to provide guarantees around the actual latency. Fig.(\ref{fig:sub-structure-conformal-prediction}) illustrates three different sub-structures: the (HJ, SS, SS) sub-structure with a corresponding \(C_{\text{(HJ, SS, SS)}}\) value of 5, the (HJ, HJ, SS) pattern with a \(C_{\text{(HJ, HJ, SS)}}\) value of 10, and the (HJ, HJ, IS) pattern with a \(C_{\text{(HJ, HJ, IS)}}\) value of 50. These $C_{\text{sub}}$ values are applied by adding and subtracting them from the predicted costs of $60, 100, 150$ respectively, resulting in adjusted ranges of $[55, 65]$, $[90, 110]$, and $[100, 200]$, respectively, thereby incorporating the conformal prediction bounds into the final cost estimations. This process ensures that the runtime behavior for each sub-structure conforms to the predicted bounds. 


% \section{Temporary store previous writing}
% \subsection{Runtime Verification\TODO{Decide Destiny}}\label{sec:runtime-verification}
% In addition to the guarantees derived from conformal prediction, we integrate robust Signal Temporal Logic (STL) with conformal prediction to perform runtime verification. Starting from equation (\ref{3.2-5}), given the actual runtime $t$ and the predicted cost 
%   $\hat{c}$ for a operation, we have the following:
% \[
% P(\rho^\phi(t) > 0) \geq 1 - \delta, \quad \text{if} \ \rho^\phi(\hat{c}) > C.
% \]

% \toshashank{Shall we mention how we calculate C again? Considering it is different from the previous one}This formula asserts that, with a high probability, the robustness of the actual runtime $t$ will satisfy the constraint $\phi$, provided that the predicted cost $\hat{c}$ is robust enough to exceed the threshold $C$. If this condition holds, it directly implies that the actual runtime will satisfy the STL constraint $\phi$. Specifically, $\rho^\phi(t) > 0$ indicates that the runtime behavior conforms to the temporal requirements imposed by $\phi$, ensuring the query plan remains within acceptable performance limits.

% \subsubsection{Violation Handling}
% During the verification, if the actual plan quality is found to be poor or significantly suboptimal, our framework classifies this as a violation. If the violation is identified, the framework discards the suboptimal plan and regenerates a new query plan. \toprof{We Would like to double check this with you. Shashank and I have a discussion today again.} Considering that a poorly optimized plan can take significantly longer to execute—on the order of minutes in large databases—compared to a trusted plan, the regeneration time, which is on the order of milliseconds, is considered acceptable. In this way, we ensure that the query engine executes only those query plans from the learned query optimizer that have been verified by conformal prediction.\toshashank{Better we have to reformulate now before the professor. To tell the difference between different plan here}


==> sections/hanwen_distribution_shift.tex <==
% \subsection{Adaptive {\cp} for Distribution Shift}

% In the preceding discussion, we have assumed that the test data $\{R^{(0)}\}$ and the calibration data $\{R^{(1)}, \dots, R^{(K)}\}$ are drawn from the same underlying distribution. Sometimes, learned components are trained in one workload and evaluated in another workload~\cite{10.14778/3583140.3583164}, which are identified as distribution shifts. To address this issue, we introduce an adaptive $\cp$ framework that dynamically adjusts to such shifts while preserving valid statistical guarantees. For the following discussion, our assumption differs slightly from Section~\ref{sec:background_cp}: $\{R^{(0)}, \dots, R^{(K)}\}$ are independent but not identically distributed. Specifically, the variable $R^{(0)} \sim \mathcal{R}$ (where $\mathcal{R}$ represents the test distribution), while $R^{(1)}, \dots, R^{(K)} \sim \mathcal{R}_{0}$ (where $\mathcal{R}_{0}$ denotes the calibration distribution). Assuming that the distributions $\mathcal{R}$ and $\mathcal{R}_{0}$ are sufficiently close, the calibration data from the training distribution $\mathcal{R}_{0}$ can still be used to bound $R^{(0)}$~\cite{zhao2024robustconformalpredictionstl}.

% \subsubsection{Distribution Shift Quantification}

% {To rigorously quantify the deviation between the training and test distributions, we employ the  $f$-divergence $D_f(D,D_0)$, which requires a convex function $f: [0,\infty) \to \mathbb{R}$ is satisfying $f(1) = 0$ as:
% \[
%     D_f(D,D_0) := \int_\mathcal{X} f\left(\frac{dD}{dD_0}\right) dD_0.
% \]
% Setting $f(x):= \frac{1}{2} |x - 1|$ yields the total variation distance: $TV(R, R_0):= \frac{1}{2} \int_x | q(x) - p(x) | dx,$ where $p(x)$ and $q(x)$ denote the probability density functions ({\pdf}s) of $\mathcal{R}$ and $\mathcal{R}_{0}$, which are empirically estimated by kernel density estimators (KDEs) with Gaussian kernels.}

% \subsubsection{Robust {\cp} under Distribution Shift}

% \textit{\textbf{Bounded shift assumption}}: The test and calibration distributions, $\mathcal{R}$ and $\mathcal{R}_{0}$, satisfy \(\mathcal{R} \in P(\mathcal{R}_0) := \{ \mathcal{R} \mid D_f(\mathcal{R}, \mathcal{R}_0) \leq \epsilon \}\), where $\epsilon$ quantifies the allowable distribution shift in $f$-divergence term.

% To handle the distribution shift under the above assumption and ensure that Equation~\ref{2.2-1} remains valid, it is sufficient~\cite{zhao2024robustconformalpredictionstl} to compute an adjusted uncertainty probability $\tilde{\delta}$ as follows:
% \[
%     \tilde{\delta}:= 1 - g^{-1}(g\left( \left( 1 + \frac{1}{K} \right) g^{-1}(1 - \delta) \right)), \tag{2}
% \]
% where $g(\beta)$ and $g^{-1}(\beta)$ is obtained by applying $f(r):= \frac{1}{2} |r - 1|$:
% \[
%     g(\beta) = \max(0, \beta - \epsilon), \quad g^{-1}(\beta) = \min(1, \beta + \epsilon).
% \]

==> sections/introduction.tex <==
\section{Introduction}
Query optimization is a critical component of Database Management Systems (DBMS), aiming to improve query processing efficiency by minimizing execution latency and resource consumption~\cite{selinger1979access,babcock2005towards}. Traditional query optimization methods, such as cost-based optimization~\cite{jayant2008identifying}, enumerate various query plans, estimate the corresponding cost, and select the most efficient one. Recently, multiple {\lqo}s have been proposed, leveraging machine learning ({\ml}) to construct complete query plans~\cite{wang2016database,kaftan2018cuttlefish}. With a few hours of training, their performance can surpass traditional query optimizers. Additionally, some {\lqo}s employ deep reinforcement learning (DQL) frameworks~\cite{sagedb_cidr,krishnan2018learning, bao, neo, marcus2018deep}, allowing them to adapt more effectively to changing data distributions and workload patterns without retraining the entire model.


% Despite their great potential, {\lqo}s have not yet been adopted in real production environments, where the top priority is ensuring the robustness and predictability of the quality of generated query plans. The opacity of {\ml} models raises concerns about their consistency and accuracy in practice. {\lqo}s sometimes may generate inconsistent or worse query plans. Executing a bad query plan can increase  actual latency 5-10x, severely impacting the overall performance of the database. Currently, a new research perspective is employing statistical methods to quantify and constrain the {\lqo}s' behavious, ensuring the predictability and reliability of {\lqo}s, which is crucial for successfully integrating {\lqo}s into real-world industrial applications. 

Despite their great potential, {\lqo}s have not yet been widely adopted in production environments~\cite{negi2021steering}, where the top priority is ensuring the predictability and robustness of generated query plans. The opacity of {\ml} models raises concerns about their consistency and accuracy, as {\lqo}s can sometimes produce inconsistent or suboptimal query plans, which are order of magnitude more expensive than the optimal plan~\cite{leis2018query, qoeval15}, severely impacting overall database performance. Currently, a new research direction involves statistical methods to quantify and constrain {\lqo}'s behavior. This approach is essential for successfully integrating {\lqo}s into real-world industrial applications.


% Hint from Sabek - Formal verification is hard … require optimal planning takes so much time, needs to be running offline …. Not suitable for runtime DB applications. Meanwhile, we have CP, an efficient statistical formal verification … provides guarantees in an efficient manner and olinestpe … has been used in many domains …. Cyberphysics …. Robotics …. However, no one used it in our db system 
Formal verification is typically regarded as a complex algorithmic process. Many approaches require extensive planning time to achieve serious guarantees, while others operate exclusively offline. In contrast, Conformal Prediction ({\cp}) \cite{cpbook05, shafer2007tutorialconformalprediction} offers a more efficient and lightweight statistical framework for formal verification, with extensions supporting runtime and offline verification \cite{cpstl23}. This method has been successfully applied in fields such as cyber-physical systems and robotics \cite{Verisig, cps2020, lindemann2022riskstochasticsystemstemporal} to ensure the reliability of critical decisions. Despite its potential, {\cp} has yet to be explored in the context of database systems.

Applying {\cp} to {\lqo} presents significant challenges, particularly because database operations are inherently time-sensitive. Thus, it is crucial to ensure that incorporating {\cp} does not introduce excessive computational overhead. Additionally, considering that {\lqo}s explore and construct query plans within an exponentially large search space, often requiring considerable planning time, a higher expectation is to integrate {\cp} into the {\lqo} planning process. This integration should ensure that the overall query plan does not result in unexpected execution latency. Achieving this goal requires designing an appropriate framework that incorporates {\cp} without disrupting the optimization flow, while still providing strong performance guarantees.


% @Shashank Not required
% Signal Temporal Logic (STL) is a formalism used to specify and reason about temporal properties of real-valued signals. It extends classical temporal logic by introducing predicates over real-valued functions of time, enabling the expression of constraints on the values of signals at specific times and over intervals. STL is particularly useful in the context of systems where continuous-time behaviors are critical, such as cyber-physical systems, robotics, and control systems. By allowing the specification of complex temporal patterns and conditions, STL provides a powerful tool for verifying system properties, ensuring safety, and optimizing performance.

% @Hanwen Update: Add first to do xxx 

% Hint -  Applying this CP in DB is very challenging ….. Because it needs to be running online verification … continue the challenges here


% In this paper, we introduce our first ….  Describe the main advantages or properties …. And we provided formal proofs for the guarantees …. We used this framework for verifying different LQO,....

% In this paper, we present the first framework that applies conformal prediction to the area of query optimization. Our framework offers two forms of validation—runtime verification and offline verification—designed for various learned query optimizers. While ensuring the lightweight nature of the model, we also provide multiple levels of granularity in the analysis. If the generated query plan passes verification, it is submitted to the query engine for execution on actual data. If it fails, the plan is handed over to a trusted query optimizer for re-generation. Learned query optimizers are traditionally considered unreliable. Our approach provides a formal verification with guaranteed confidence and prevents the slow execution of untrustworthy or unpredictable query plans in the query engine. Our method supports the deployment of learned query optimizers in real-world production environments. We also provide rigorous theoretical proof to ensure the correctness of our approach. The conformal prediction framework is a lightweight and general formal verification method that is not only applicable to learned query optimizers but also promising for future expansion to other learned components in database systems. 
In this paper, we present the first general framework that applies {\cp} to {\lqo}. Our framework provides latency guarantees and runtime verification for {\lqo}s. The {\cp}-based latency guarantee employs {\cp} to offer user-controlled guaranteed ranges for the actual latency of constructed partial plans with a user-defined confidence level. The {\cp}-based runtime verification uses {\cp} to detect performance constraint violations during the plan construction process, defining a violation handling mechanism to address these detected issues. Additionally, we propose a {\cp}-guided heuristic algorithm to enable the current {\lqo} to generate more optimal query plans within shorter timeframes. We also provide rigorous theoretical proof to ensure the correctness of our approach, facilitating the deployment of {\lqo}s in real-world environments. Our work demonstrates that {\cp} holds promising potential for future applications across other learned components in database systems.


% Our experimental results demonstrate the successful identification of tight performance boundaries for the IMDB and TPCH workloads across multiple learned query optimizers, including Balsa, Lero, and TreeLSTM. In particular, we observed that the conformal prediction functions provides effective thresholds for estimating performance. Additionally, we identified significant thresholds for frequently used operation sequences, which were prominent in the Balsa optimizer. These performance boundaries were formally verified, achieving a high guarantee level, indicating that the conformal score consistently remained below the established thresholds in the majority of cases.

% Our experimental results on the JOB and TPC-H workloads first confirm the correctness of applying {\cp} to query optimization by verifying empirical coverage. We then demonstrate the successful latency guarantees across multiple {\lqo}s, including Balsa, Lero, and RTOS, all aligning with theoretical expectations. In runtime verification, we show that our {\cp}-based methods accurately detect violations, and our violation handling methods improve overall execution latency by 12,030.1ms among 7 violation queries. With the {\cp}-guided algorithm, our approach enhances 33\% queries' plan quality even from basically trained {\lqo} and also achieve 9.96\% overall planning latency improvement on all test queries. For well-trained {\lqo} we can also find better quality and faster planning queries. These comprehensive experiments substantiate the correctness and effectiveness of our {\cp} framework.

Our experimental results on the JOB and TPC-H workloads first confirm the correctness of applying {\cp} to {\lqo} by verifying empirical coverage. We then demonstrate the effectiveness of latency guarantees across multiple {\lqo}s, including Balsa, Lero, and RTOS, all aligning with theoretical expectations. In runtime verification, we show that our {\cp}-based methods accurately detect violations, and our violation handling strategies reduce overall execution latency by 12,030.1 ms across 7 violation queries. Using the {\cp}-guided algorithm, our approach improves plan quality in 33\% of queries from a moderately trained {\lqo}, achieving an additional 9.96\% reduction in overall planning latency across all test queries. For well-trained {\lqo}s, we also observe better plan quality and faster query planning with our {\cp}-guided algorithm. These comprehensive experiments substantiate the correctness and effectiveness of our {\cp} framework.



% Our experimental results demonstrate that we successfully identified tight performance boundaries for the IMDB and TPCH workloads across multiple learned query optimizers, including Balsa, Lero, and TreeLSTM. Specifically, for the JOB workload, we observed an average threshold of 2745 ms using the \(|x_{\text{obs}} - X|\) conformal function, and 2619 ms with the \(x_{\text{obs}} - X\) conformal function. Furthermore, we obtained an average threshold of 3056 ms for the operation sequence (Hash join, Hash join, Seq scan), which was the most frequently used pattern by Balsa. These performance boundaries were formally verified, with a guarantee of 0.9, indicating that the conformal score remained below the threshold in 90\% of the cases.

In summary, our contributions are as follows: 
\begin{itemize}
    \item We are the first to formulate the Learned Query Optimizer ({\lqo}) verification as a Conformal Prediction ({\cp}) problem.
    \item We develop {\cp}-based Latency Guarantees for {\lqo}s to provide a user-defined confidence level of guaranteed range for the actual latency of query plans.
    \item We design {\cp}-based runtime verification and a violation handler for white-box {\lqo}s, which detect and address unexpected long-latency query plans before execution.
    \item We introduce a {\cp}-guided query optimization algorithm that can enhance both the query plan quality and the planning time from a trained {\lqo}.
    \item Our experimental evaluation across three prototypes and two workloads demonstrates the correctness and effectiveness of our {\cp}-based framework for {\lqo}s.
\end{itemize}



==> sections/prototype.tex <==
\section{Prototype Implementations (Add a double column graph)}
\subsection{Balsa}
Balsa is a learned query optimizer designed to replace traditional heuristic-based optimizers by utilizing a learned model to generate query execution plans. Given an input SQL query, Balsa constructs an execution plan using a beam search approach. Beam search ensures that at least one valid execution plan is produced by the end of the search process. At each step, Balsa employs a predictive model to estimate the cost of performing each join operation. The most promising joins are added to the beam, and the number of nodes expanded at each step is determined by the predefined beam size. Balsa's exploration-exploitation strategy then selects the subsequent step for query plan construction.

Conformal prediction integrates seamlessly into this framework by providing rigorous guarantees on the predicted performance of each join. After Balsa generates a prediction for the cost of a join, conformal prediction can be used to validate the accuracy of these predictions, offering a statistically reliable interval within which the actual runtime is expected to fall. By leveraging sub-structure level conformal prediction, Balsa can select query plans that strike a balance between exploration and exploitation, thus avoiding overly conservative or overly risky plans. This allows Balsa to ensure that the selected plan does not deviate significantly from the predicted cost estimates, improving both the robustness and reliability of the query optimization process.

\begin{figure}[ht]
\centering 
\includegraphics[width=\linewidth]{figures/Prototypes/Balsa.png}
\caption{Balsa Implementation Prototype} 
\label{fig:Quantile inforamtion for 100 iterations}
\end{figure}

\subsection{Lero}
Instead of using a machine learning model to predict latency at the sub-plan level and then constructing the entire query plan, Lero generates multiple candidate query plans through a native query optimizer and introduces a learned oracle capable of ranking these plans. This learned oracle utilizes a pairwise comparison approach, where two plans are compared at a time, and it predicts which one is more efficient. This method requires fewer training samples and less training time compared to pointwise approaches, which directly predict execution efficiency before performing comparisons. Ultimately, Lero outputs the top-ranked plan as the final result.

Since Lero's plan generation process does not expose visible intermediate stages, we apply conformal prediction after the plan is generated. First, Lero generates a query plan, and then we apply conformal prediction while the plan is analyzed in PostgreSQL. At this stage, the predicted cost \(\hat{c}\) is available, and we use conformal prediction to obtain the prediction region for the actual runtime \(t\), based on the predicted cost \(\hat{c}\).

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/Prototypes/old-lero-prototype.png}
    \caption{CP4Lero Implementation Prototype\TODO{Will this contradict to the core framework? Because we have plan right now}]}
    \label{fig:lero-prototype}
\end{figure}


\subsection{RTOS}
RTOS represents a distinct branch of learned query optimization focused on join order selection. RTOS leverages a Reinforcement Learning framework in conjunction with Graph Neural Networks (GNNs) to effectively capture the structural information of query plans. Unlike earlier learned optimizers that primarily encode join trees using fixed-length vectors, RTOS employs a Tree-structured Long Short-Term Memory (Tree-LSTM) model, which is capable of adapting to changes in the database schema. Through its machine learning model, RTOS generates a join ordering, serving as a hint for the query optimizer to construct the entire query plan.

During the actual query plan construction, we can apply conformal prediction to evaluate the quality of the predicted join ordering. The predicted cost \(\hat{c}\) reflects RTOS's join order selection effectiveness. Based on \(\hat{c}\), we then proceed to perform both guarantees and runtime verification, ensuring the robustness and efficiency of the query execution.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/Prototypes/RTOS.png}
    \caption{CP4RTOS Implementation Prototype}
    \label{fig:cp4rtos}
\end{figure}


==> sections/related-work.tex <==
\section{Related Work}
%% As is from the STL paper
% \textbf{Learned Query optimization.}
% In recent work, Neo~\cite{neo} and Balsa~\cite{balsa} propose end-to-end learned solutions for query optimization. Neo introduces a novel query encoding technique, Tree Convolution, to implicitly capture correlations. It relies on deep neural networks to generate complete query execution plans. Balsa tries not to rely on learning from an existing expert optimizer by adopting a simulation-to-reality learning framework. Balsa performs beam search, maintaining multiple top candidate partial plans and continuously exploring them. The transparent planning feature of Balsa allows for the integration of conformal prediction, offering enhanced reliability in query optimization.

% Lero~\cite{zhu2023lero}, diverging from traditional methods that predict cost or latency, builds a machine-learning model to perform pairwise plan comparisons. Lero improves end-to-end performance by learning the differences between plan pairs and efficiently exploring plans.

% Another branch of learned query optimizer focuses on join order selection, utilizing various methods to encode a join tree. DQ~\cite{krishnan2018learning} and ReJOIN~\cite{marcus2018deep} use fixed-length vectors to encode join trees, while RTOS~\cite{yu2020reinforcement} introduces Tree-LSTM, which supports modifications to the database schema. In our analysis, we selected RTOS as the representative method for join-order query optimization.

% Bao~\cite{bao} learns to generate per-query hints based on workloads, data, and schema, thereby improving query planning within the query optimizer.

\textbf{Learned Query Optimization.}
Recent works have introduced a range of end-to-end learned solutions for query optimization. Neo~\cite{neo} and Balsa~\cite{balsa} represent two notable approaches within this field. Neo introduces a novel query encoding technique, Tree Convolution, to implicitly capture correlations and relies on deep neural networks to generate complete query execution plans. In contrast, Balsa reduces reliance on traditional expert optimizers by employing a simulation-to-reality learning framework. Using beam search, Balsa maintains multiple top candidate partial plans and continuously explores them. This transparent planning feature enables the integration of conformal prediction, enhancing the reliability of query optimization. 

Lero~\cite{zhu2023lero} takes a unique approach by constructing a machine learning model that performs pairwise plan comparisons rather than traditional cost or latency prediction. By learning to differentiate between plans, Lero can efficiently explore and improve query performance end-to-end. Another line of learned query optimizers, exemplified by DQ~\cite{krishnan2018learning}, ReJOIN~\cite{marcus2018deep}, and RTOS~\cite{yu2020reinforcement}, focuses specifically on join order selection, employing various methods to encode join trees. DQ and ReJOIN utilize fixed-length vectors to represent join trees, while RTOS introduces Tree-LSTM to accommodate changes in database schema. For our analysis, RTOS serves as the representative method for join-order query optimization. Additionally, Bao~\cite{bao} contributes to this field by learning to generate per-query hints based on workloads, data, and schema, thereby improving query planning within the optimizer. Together, these approaches showcase the versatility and potential of learned techniques in enhancing database query optimization.


% \textbf{Conformal prediction.} {\cp} was introduced by Vovk et al.~\cite{inbook} and Shafer and Vovk~\cite{shafer2007tutorialconformalprediction}, provides a statistical framework to quantify the uncertainty of predictions without relying on assumptions about the data distribution. Several works have explored conformal prediction in distribution-agnostic settings~\cite{angelopoulos2022gentleintroductionconformalprediction, fontana2023conformal, lei2018distribution}, providing guarantees even in unpredictable environments. Extensions to time-series data~\cite{cpcovshift19, cauchois2020robust} and applications in runtime verification have been demonstrated, such as verifying Signal Temporal Logic (STL) specifications for real-time systems~\cite{lindemann2023conformalpredictionstlruntime}.

% \textbf{Conformal Prediction.} {\cp}, introduced by Vovk et al.~\cite{inbook} and Shafer and Vovk~\cite{shafer2007tutorialconformalprediction}, provides a statistical framework for quantifying the uncertainty of predictions without making assumptions about the data distribution. Several studies have explored conformal prediction in distribution-agnostic settings~\cite{angelopoulos2022gentleintroductionconformalprediction, fontana2023conformal, lei2018distribution}, providing robust guarantees even in unpredictable environments. Extensions of {\cp} to time-series data~\cite{cpcovshift19, cauchois2020robust} and applications in runtime verification have also been demonstrated, such as the verification of Signal Temporal Logic (STL) specifications for real-time systems~\cite{lindemann2023conformalpredictionstlruntime}.


% More recently, conformal prediction has been applied to policy evaluation in reinforcement learning~\cite{foffano2023conformaloffpolicyevaluationmarkov, taufiq2022conformal}, time-series forecasting~\cite{NEURIPS2021_312f1ba2}, and outlier detection~\cite{Bates_2023}. It has also been used to track risks in evolving data streams~\cite{podkopaev2022trackingriskdeployedmodel} and to detect change points in time-series data~\cite{Vovk_2021, pmlr-v60-volkhonskiy17a}. These varied applications highlight the flexibility and importance of conformal prediction in providing reliable performance guarantees across different domains.

\textbf{Conformal Prediction.} {\cp}, introduced by Vovk et al.~\cite{cpbook05} and Shafer and Vovk~\cite{shafer2007tutorialconformalprediction}, provides a robust statistical framework for quantifying prediction uncertainty. Extensive research has explored the application of conformal prediction in distribution-agnostic settings~\cite{angelopoulos2022gentleintroductionconformalprediction, fontana2023conformal, lei2018distribution}, delivering reliable performance guarantees even in non-stationary environments. Additionally, extensions of {\cp} have been applied to time-series data~\cite{cpcovshift19, cauchois2020robust} and runtime verification, such as verifying Signal Temporal Logic (STL) specifications in real-time systems~\cite{cpstl23}. Besides, conformal prediction has been adapted for policy evaluation in reinforcement learning~\cite{foffano2023conformaloffpolicyevaluationmarkov, taufiq2022conformal}, time-series forecasting~\cite{NEURIPS2021_312f1ba2}, and outlier detection~\cite{Bates_2023}. It has also been employed to monitor risks in evolving data streams~\cite{podkopaev2022trackingriskdeployedmodel} and detect change points in time-series data~\cite{Vovk_2021, pmlr-v60-volkhonskiy17a}. These diverse applications underscore the flexibility and significance of conformal prediction in ensuring reliable performance across various domains.


% \textbf{Signal Temporal Logic.} Conformal prediction was used for verification of STL properties in by learning a predictive model of the STL semantics. For reachable set prediction, the authors in [69–71] used conformal prediction to quantify uncertainty of a predictive runtime monitor that predicts reachability of safe/unsafe states. However, the works in [68–71] train task-specific predictors while we use task-independent trajectory predictors to predict future system states from which we infer information about the satisfaction of the task. This is significant as no expensive retraining is required when the specification changes.

